Learning Ising models from one or multiple samples

There have been two separate lines of work on estimating Ising models: (1) estimating them from multiple independent samples under minimal assumptions about the model's interaction matrix; and (2) estimating them from one sample in restrictive settings. We propose a unified framework that smoothly interpolates between these two settings, enabling significantly richer estimation guarantees from one, a few, or many samples. Our main theorem provides guarantees for one-sample estimation, quantifying the estimation error in terms of the metric entropy of a family of interaction matrices. As corollaries of our main theorem, we derive bounds when the model's interaction matrix is a (sparse) linear combination of known matrices, or it belongs to a finite set, or to a high-dimensional manifold. In fact, our main result handles multiple independent samples by viewing them as one sample from a larger model, and can be used to derive estimation bounds that are qualitatively similar to those obtained in the afore-described multiple-sample literature. Our technical approach benefits from sparsifying a model's interaction network, conditioning on subsets of variables that make the dependencies in the resulting conditional distribution sufficiently weak. We use this sparsification technique to prove strong concentration and anti-concentration results for the Ising model, which we believe have applications beyond the scope of this paper.

==> additional-examples.tex <==
\section{Additional examples}
\label{app:addnl-examples}

\subsection{Multiple networks, each containing sufficiently many unique friendships}

Here is an example when the theorem can be applied: assume we have $k$ different types of connections, corresponding to graphs $([n],E_1),\dots,([n],E_k)$ with incidence matrices $J^1,\dots,J^k$, namely, $J^{s}_{ij} = 1$ if $(i,j) \in E_s$ and otherwise $J^s_{ij} = 0$. 
Assume that each connection graph has an unknown influence $\beta_i$, such that the interaction matrix of the Ising model is $J^* = \sum_i \beta_i^* J^i$. For all $s$, let
\[
\Lambda_s = E_s \setminus (\bigcup_{t \in [n]\setminus\{s\}} E_t),
\]
and let $\lambda_s = |\Lambda_s|$ which equals the number of edges unique to $E_s$.
Assume that $\hat J = \sum_s \hat\beta_s J^s$. Then,
\[
\sum_s \lambda_s (\hat\beta_s - \beta_s^*)^2 \le \|\hat J - J^*\|_F^2,
\]
and particularly,
\[
\|\hat \beta_s - \beta_s^*\|_2
\le \frac{\|\hat J - J^*\|_F}{\sqrt{\min_s \lambda_s}}.
\]

To prove the above, we substitute $\beta:=\hat\beta - \beta^*$ and calculate
\[
\|\sum_s \beta_s J^s\|_F^2 
= \sum_{i,j\in[n]}(\sum_{s\in[k]} \beta_s J^s_{ij})^2
\ge \sum_{i,j\in[n]}\sum_{s \in [k]} \sum_{(i,j) \in \Lambda_s}\beta_s^2
= \sum_s \lambda_s \beta_s^2.
\]

\subsection{Samples from a network with an additional temporal correlation}

\section{Can we get a tight bound on the partition function?}
We essentially have to compare $x^\top A x$ and $x^\top A^2 x$. Decompose into the singular values...

Use the result from inference in Ising models, where they compare $x$ to $Ax$, and in fact say that $x \approx \tanh (Ax)$.

Perhaps replace the maximum over sub-samples by a simple bound of $\|Ax\|_2 + 1$. We actually already have this: the derivative is bounded in terms of the value of $\|Ax\|_2$. By the triangle inequality and using their trick, we get that $x^\top A x$ cannot be much larger than $x^\top A^\top A x$.

So, in fact, we get a control as a function of $x^\top A x$: if it's large then we can learn, and otherwise, we cannot!

Rate can be \emph{certified} by $x^\top A x$: if this value is large, then we know that we've learned well! Even if we don't have the guarantee on the partition function, that was needed in "inference".

Have an improved statement over inference, that only requires one sided bound on the partition function.

Say we have one matrix $J$ and that the true parameter is $\beta^*$. Let $F(\beta)$ denote the log partition function.

We have the following lemma:
\begin{lemma}
	
\end{lemma}
\begin{proof}
	First of all, let $J$ denote the true matrix.
	And $r > 0$. Then, we have that
	\[
	\Pr_{J}[x^\top J x < r]
	= \Pr[e^{-x^\top J x/2} < e^{-r/2}]
	\le \exp(\frac{1}{2}r - F_n(J))
	\]
	Next, we compare $x^\top J x$ with $x^\top J^\top J x$, and show that $x^\top J^\top J x \ge C x^\top J x$. Indeed, assume that $x^\top J x \ge x^\top J^\top J x$, otherwise we're done. Then, we derive that $x^\top J^\top J x \ge \tanh(x^\top J^\top) J x$, since in the inner product we have a sum of $n$ products, and in each one of them we have an inequality. Next, we have that 
	\[
	|\tanh(x^\top J^\top) J x - x^\top J x| \le C \|Jx\|_2,
	\]
	from the above inequality. We derive that
	\[
	\|Jx\|_2^2 
	\ge |\tanh(x^\top J^\top) Jx| 
	\ge |x^\top J x| - \|Jx\|_2.
	\]
	We have an inequality: $x^2 + x - t \ge 0$, hence we derive that the solution are
	\[
	\frac{-1\pm \sqrt{1+4t}}{2}.
	\]
	Since we have the positive inequality, we get that $\|Jx\|_2 \ge \Omega(-1 + \sqrt{1+4t})$.
	
	So, we derive that the strong convexity is at least $x^\top J x$, namely, $\partial^2\varphi(J)/\partial J^2 \ge F_n(J)/2$. And the derivative is a square root of that. Therefore, $\|\hat{J} - J\| \le \sqrt{1/F_n} \|J\|$.
	Now, in terms of $\beta$, it means that the rate is bounded by $\beta^* /\sqrt{F_n}$.
	
	Notice what happens under Dobrushin's condition with a small $\beta$. In the Frobenius shape, the error would be $1/\|J\|_F$. The partition function is $F(A) = \|A\|_F^2$, hence for our case it is $\beta^2 \|J\|_F^2$. And, if we take $\beta / \|A\|_F^2$, we have $1/\sqrt{\|J\|_F}$.
\end{proof}
\yuval{If we can show that the partition function is lower bounded by the Frobenius norm, then we can show that our theorem is tight under Dobrushin's condition. Additionally, this will show that the Frobenius lower bound is weaker than the partition function bound. Indeed, this is true because we can learn up to a rate of $1/\|A\|_F$ under Dobrushin's condition, and otherwise it wouldn't be possible! Also we can check the proof of inference in Ising models.}

Can we lower bound the partition function by the Frobenius norm? Use the variance of $x^\top A x$.

\yuval{Find specific applications. For example, Curie Weiss (although it's known), or, random graph in high temperature.}

\subsection{One parameter}

In the one-parameter setting, using the same proof as Theorem\yuval{REF- multi-parameters}, we can perform a more fine-grained analysis. Here we assume a known interaction matrix $J \in M_{n\times n}(\mathbb{R})$ and an unknown parameter $\beta^*$, such that $x \sim P_{\beta^* J}$. As in Theorem\yuval{REF} we assume that $\|\beta^*J\|_\infty$ is at most some constant, and without loss of generality, $\|J\|_\infty = 1$ and $\beta^* = O(1)$ (possibly $\beta > 1$). We analyze the pseudo log likelihood estimator:
\begin{theorem}[informal]
	Assume that $\|J\|_\infty = 1$, and let $\hat \beta$ denote the pseudo likelihood estimator of $\beta^*$. Then, with high probability over $x$,
	\[
		|\hat\beta-\beta^*|
		\le O(\|Jx\|_2^{-1} \sqrt{\log\log n})
		\le O(\beta^* Z_{\beta^*J}^{-1/2}\sqrt{\log\log n})
		\le O(\|J\|_F^{-1}\sqrt{\log \log n}).
	\]
\end{theorem}
We note that this nearly generalizes and improves all the prior work.
Chatterjee \yuval{cite} was the first to study this problem, and he gave a rate of $1/\sqrt{n}$ assuming that $Z_{\beta^*J} \ge $

\section{Parameter-specific learning}

\section{People to remember to cite}

Aryeh Kanterovich

Valiant?

Dheeraj

==> algorithm.tex <==
\begin{lemma}\label{lem:optimization}
	There exists an algorithm that outputs $\hat{J}$ satisfying $\hat{J} \in V$ and $\|\hat{J}\|_\infty \le 2M$, such that 
	$$
	\varphi(\hat{J}) \le \varphi(J^*) + k
	$$
	
	and runs in time $O(kn^4)$.
\end{lemma}
\begin{proof}
The algorithm essentially solves the constrained optimization
problem described in ~\ref{eq:pmle}.
To design the optimization algorithm, it will be more 
convenient to work with a specific base of matrices
that span $V$. For this reason,
let $\{A_1,\ldots,A_k\}$ be a fixed orthonormal basis of $V$ with
respect to the inner product induced by the Frobenius norm.
Then, each $J \in V$ can be uniquely written in the form 
$$
J = \sum_{i=1}^k \beta_i A_i
$$
We use the notation $\pmb{\beta} = (\beta_1,\ldots,\beta_k)$
and $A_{\pmb{\beta}} = \sum_{i=1}^k \beta_i A_i$.
Thus, minimizing $\varphi(J)$ subject to $J \in \mathcal{J}$
is the same as minimizing 
$$
\psi(\pmb{\beta}) = \varphi(A_{\pmb{\beta}})
$$
subject to the constraint $\|A_{\pmb{\beta}}\|_\infty \le M$.
Thus, in order to solve ~\ref{eq:pmle}, we can equivalently
solve 
\begin{equation}\label{eq:alt_pmle}
    \arg\min_{\pmb{\beta}:\|A_{\pmb{\beta}}\|_\infty \le M}
    \psi(\pmb{\beta})
\end{equation}
One way to solve this is to use constrained
optimization.
 However, we would like to avoid the complicated
projection procedure associated with this strategy.
Instead, we will solve the following regularized
optimization problem:
$$
\arg\min_{\pmb{\beta}} \lp(\psi(\pmb{\beta})+ \lambda\max(0,\|A_{\pmb{\beta}}\|_\infty - M)\rp)
$$
Set $h(\pmb{\beta}) = \psi(\pmb{\beta})+ \lambda\max(0,\|A_{\pmb{\beta}}\|_\infty - M)$.
We will describe a way to pick $\lambda$ shortly after.
Denote by $\pmb{\beta}_1$ the solution of this optimization problem and by $\pmb{\beta}^*$ the one corresponding to $J^*$.
Also, suppose the algorithm outputs a point $\hat{\pmb{\beta}}$
for accuracy $\epsilon = k$.
We will prove that
$\|A_{\pmb{\beta}_1}\|_\infty, \|A_{\hat{\pmb{\beta}}}\|_\infty \le 3M$.
First, by equation~\ref{eq:pmleform}
is is clear \vardis{give more explanation} that 
$$
\psi(\pmb{\beta}) \leq Mn
$$
for all $\pmb{\beta}$ satisfying $\|A_{\pmb{\beta}}\|_\infty \le 3M$. Hence, by choosing $\lambda = n$,
it is clear that for all $\pmb{\beta}$ such that 
$\|A_{\pmb{\beta}}\|_\infty \ge 3M$, 
$$
\max(0,\|A_{\pmb{\beta}}\|_\infty - M) \ge 2Mn.
$$
This means that the optimal point $\pmb{\beta}_1$ lies in the set
$\{\pmb{\beta}:\|A_{\pmb{\beta}}\|_\infty \le 2M\}$.
Moreover, we have
$$
h(\hat{\pmb{\beta}}) - h(\pmb{\beta}_1)\le k \le Mn
\implies h(\hat{\pmb{\beta}}) \le 2Mn
\implies \|A_{\hat{\pmb{\beta}}}\|_\infty \le 3M
$$
As for the guarantee of the algorithm, we notice that:
$$
\psi(\hat{\pmb{\beta}}) \leq h(\hat{\pmb{\beta}})
\leq h(\pmb{\beta}_1) + k
\le h(\pmb{\beta}^*) + k = \psi(\pmb{\beta}^*) + k
$$
since $\|A_{\pmb{\beta}}^*\|_\infty \leq M$.
Thus, if we denote by $\hat{J} = A_{\hat{\pmb{\beta}}}$,
we conclude that:
$$
\varphi(\hat{J}) \le \varphi(J^*) + k
$$
which is what we wanted to prove.
It remains now to argue about the computational complexity
of the procedure. The algorithm we will use is subgradient descent, which performs reasonable well when the subgradient is
upper bounded.
The following Theorem can be found in \cite{bubeck2015convex}.
\begin{theorem}[\cite{bubeck2015convex}]\label{t:gd}
Suppose $f$ is a convex function with minimum $x^*$ and $g \in \partial f$ is
a subgradient such that $\|g\| \le L$. Suppose we are running the
following iterative procedure:
$$
x_{t+1} = x_t - \eta g(x_t)
$$
with $\|x_1 - x^*\| \le R$.
If we choose $\eta = R/(L\sqrt{t})$
then 
$$
f\lp(\frac{1}{t} \sum_{i=1}^t f(x_i)\rp) - f(x^*) \leq \frac{RL}{\sqrt{t}}
$$
\end{theorem}
Hence, if we want accuracy $\epsilon = k$, we need to run the algorithm
for $t = O(R^2L^2)$ iterations. 
We now argue that both $R$ and $L$ are polynomially
bounded in our case. 
First of all, it is easy to see that $\partial \psi(\pmb{\beta})/\partial \beta_i \le Mn$.
\vardis{more explanation here}
Also, for the function $\max(f,g)$ a suitable subgradient
is any of the gradients of $f$ or $g$.
The term $\max(0,\|A_{\pmb{\beta}}\|_\infty - M)$ features
a hidden maximum operation inside the infinity norm.
This means that we can calculate the subgradient of just
one of the absolute row sums of $\|A_{\pmb{\beta}}$.
However, this is just a sum of absolute values of $n$ variablew. We conclude that for the term $\lambda\max(0,\|A_{\pmb{\beta}}\|_\infty - M)$ a bound for the subgradient $g_i$ is just $\lambda$.
Hence, the total norm of the subgradient of $h$ is bounded by
$\sqrt{k}Mn$. Furthermore, calculating these subgradients clearly
takes $O(n)$ time. 
Finally, we have 
$$
\|x_1 - \pmb{\beta}^*\| = \|A_{x_1} - A_{\pmb{\beta}^*}\|_F \leq \sqrt{n}\|A_{x_1} - A_{\pmb{\beta}^*}\|_\infty \le M\sqrt{n}
$$
Hence, after $t = O(kn^4)$ rounds we have the desired result.
\end{proof}

==> chaining-bounds.tex <==
\section{In progress - improved bounds via chaining}
\yuval{I'm changing it a bit at the moment}

We would like to use Dudley type integral to improve the bound and generalize to arbitrary estimation problems. For convenience we assume Dobrushin's condition, however, this can be generalized using conditioning. More concretely, we have some convex set $\J$ containing interaction matrices with infinity norm bounded by $O(1)$, and there is an unknown interaction matrix $J^* \in \J$ where the sample is drawn from. We will bound the difference $\hat{J}-J^*$ in terms of the norm $\|\cdot\|_\kappa$ defined by
\[
\|A\|_\kappa = \max(\|A\|_F, \|\E[Ax]\|_2).
\]
We will obtain the rate as a function of the geometry of the set $\J$ and of $J^*$. Concretely, define the following set of directions, corresponding to a sphere of radius $t$ around $J^*$ 
\[
\mathcal{A}_t 
= \lp\{
A \in M_{n\times n}(\mathbb{R}) \colon 
\|A\|_\kappa \le t, J^* + A \in \J
\rp\}.
\]
We would like to bound the first and second derivatives of the MPLE with respect to matrices $A \in \A_t$. We have the following statement, and recall that $\varphi(J)$ denotes the log pseudo likelihood of the matrix $J$ with respect to the obtained sample. 
\begin{lemma}\label{lem:select-t}
Fix $t > 0$, fix the sample $x$ and assume that for all $A \in \A_t$, $x^\top A^2 x \ge \E[x^\top A^2 x]/2$.
Then, 
\begin{equation}\label{eq:922}
\|\hat{J} - J^*\|_\kappa
\le O\lp(\max\lp(t,  
    \frac{1}{t}\max_{A \in \A_t} \lp| \frac{\partial \varphi(J^*)}{\partial A}\rp|
\rp)\rp).
\end{equation}
\end{lemma}
\begin{proof}
\yuval{to fix proof}
Assume that $\|\hat{J} - J^*\|_\kappa>t$. Then, from convexity of $\J$, 
\[
A_\Delta := \frac{\hat{J}-J^*}{\|\hat{J}-J^*\|_\kappa} \in \mathcal{A}_t.
\]
since 
$$
J^* + t\frac{\hat{J}-J^*}{\|\hat{J}-J^*\|_\kappa} = 
\lp(1 - \frac{t}{\|\hat{J}-J^*\|_\kappa}\rp) J^* +  \frac{t}{\|\hat{J}-J^*\|_\kappa}\hat{J}
$$
and both $J^*, \hat{J} \in \mathcal{J}$.
The error is bounded in terms of the ratio between the first and second derivatives of $\varphi(J)$ with respect to $A_\Delta$. The second derivative is constant, from the assumption on $x^\top A^2 x$, hence we derive the desired result.
\end{proof}

Given the above result, it suffices to show bound on the first and second derivatives, with respect to $\A_t$. First, some preliminaries. Given a family $\mathcal{Z}$ of random variables, it can be viewed as a metric space with respect to the $\psi_1$ norm differenence, namely $\mathrm{dist}(Z,Z') = \|Z-Z'\|_{\psi_1}$. Then, we can present the covering number $N(\mathcal{Z}, \epsilon B_{\psi_1})$ as the covering number of $\mathcal{Z}$ at scale $\epsilon$ with respect to the metric $\psi_1$.
A Dudley-type integral states the following:
\begin{lemma}
\[\E[\sup_{\mathcal{Z}}Z]
\le C\int_{0}^\infty \log N(\mathcal{Z}, \epsilon B_{\psi_1}) d\epsilon.\]
\end{lemma}
\yuval{To Vardis: a proof should definitely be appearing somewhere in literature. However, it may be a good exercise for you to work out the details, modifying the proof of Dudley's integral (for subGaussian differences)}

In our application, to bound the first derivative, we use the fact that
\[
\lp\| \frac{\partial\varphi(J^*)}{\partial A} - \frac{\partial \varphi(J^*)}{\partial B}\rp\|_{\psi_1}
= \lp\|\frac{\partial \varphi(J^*)}{\partial (A-B)} \rp\|_{\psi_1}
\le C\|A-B\|_\kappa.
\]
Then, the $\psi_1$ covering numbers of $\{\frac{\varphi(J^*)}{\partial A} \colon A \in \A_t\}$ are bounded in terms of the $\kappa$. In particular, define
\[
F_t = \int_0^\infty \log N(\A_t, \epsilon B_\kappa),
\]
where $B_\kappa$ is the unit ball of the norm $\|\cdot\|_\kappa$.
Then, with high probability,
\[
\sup_{A \in \A_t} \lp| \frac{\partial \varphi(J^*)}{\partial A}\rp| \le C F_t.
\]

To show concentration of the second derivative, we use the fact that for $A,B \in \A_t$,
\begin{align*}
&\|x^\top A^2 x - x^\top B^2 x\|_{\psi_1}
\le C\|A^2-B^2\|_F + C\| \E[(A^2-B^2)x] \|_2.
\end{align*}
To bound the first term:
\begin{align*}
&\|A^2-B^2\|_F
= \|(A-B)(A+B) + (A+B)(A-B)\|_F/2
\le \|(A-B)(A+B)\|_F/2 + \|(A+B)(A-B)\|_F/2 \\
&\le \|A-B\|_F \|A+B\|_2
\le \|A-B\|_F (\|A\|_2 + \|B\|_2)
\le C\|A-B\|_F,
\end{align*}
using the fact that for all $A \in \A_t$, $\|A\|_2\le O(1)$. 
To bound the second term:
\begin{align*}
    \| \E[(A^2-B^2)x] \|_2
\end{align*}

Again, we can use Forbenius covering numbers with respect to $\mathcal{A}_t$ to show uniform concentration. We derive that with high probability
\begin{equation}\label{eq:32}
\sup_{A \in \A_t} \lp|\frac{\partial^2\varphi(J^*)}{\partial A^2} - \E \frac{\partial^2\varphi(J^*)}{\partial A^2}\rp|
\le C F_t/t.
\end{equation}
We derive the following rate:
\begin{theorem}
Let $t^*$ denote the solution of $F_t = t$. Then, with high probability,
\[
\|\hat{J}-J^*\|_F \le C t^*.
\]
\end{theorem}
\begin{proof}
First of all, notice that $F_t$ is monotonically non-increasing, hence there exists a unique solution to $F_t = t$. Indeed, for any $t_2>t_1$, $\A_{t_2}\subseteq A_{t_1}$ by convexity of $\J$, hence $F_{t_2} \le F_{t_1}$.

Notice that there exists a constant $c_1$ such that for all $A \in \A_t$:
\[
\E \frac{\partial^2\varphi(J^*)}{\partial A^2} \ge c_1.
\]
Let $C$ denote the constant in \eqref{eq:32}. And let $t' = \max(t^*,2Ct^*/c_1)$. Then, w.h.p, for all $A \in \A_{t'}$,
\[
\lp|\frac{\partial^2\varphi(J^*)}{\partial A^2} - \E \frac{\partial^2\varphi(J^*)}{\partial A^2}\rp|
\le C F_{t'}/t'
\le c_1 F_{t'}/(2t^*)
\le c_1 F_{t^*}/(2t^*)
= c_1/2
\le \E \frac{\partial^2\varphi(J^*)}{\partial A^2}/2,
\]
using the fact that $t'\ge t^*$ and the monotonicity of $F_t$.
We derive that 
\[
\frac{\partial^2\varphi(J^*)}{\partial A^2}
\ge \E \frac{\partial^2\varphi(J^*)}{\partial A^2}/2,
\]
hence we can apply Lemma~\ref{lem:select-t} with $t'$. Since the maximal derivative within $A_{t'}$ is bounded by $C' F_{t'} \le C' F_{t^*}$ with high probability, the proof follows.
\end{proof}

To apply the above bounds for the setting in the original paper, which corresponds to a linear combination of $k$ matrices, use $t^* \le Ck$. The Forbenius covering numbers equal $N(\A_t, \epsilon B_F) \le (3/\epsilon)^{k-1}$ for $\epsilon < 1$ and $N(\A_t, \epsilon B_F) \le 1$ for $\epsilon \ge 1$, hence $F_t \le O(k)$ for all $t$.


\subsection{Mixed bounds utilizing both the spectral and Forbenius norm}

\subsection{Further improvements - TBD}
First, to find bounds that utilize that the concentration has both subgaussian and subexponential terms.

Secondly, to use general loss functions. Then, $A_t$ should correspond to the norm of a sphere with respect to a different metric. This might require too many details..

==> estimating-parameters.tex <==
\section{Estimating the Parameters} \label{sec:estimating-beta}
In this section, we show how Theorem~\ref{thm:informal-main} can be used to derive rates on the estimated parameters.
Notice that the ratio $\lambda:= \inf_{\beta \ne 0} \|\sum_i \beta_i J_i\|_F/\|{\beta}\|_2$, which corresponds to the minimal singular value of the operator $\beta \mapsto \sum_i \beta_i J_i$ between the Hilbert spaces $(\mathbb{R}^k, \|\cdot\|_2)$ and $(M_{n\times n}(\mathbb{R}),\|\cdot\|_F)$, captures the following guarantee in estimating $\beta$: $\|\beta^*-\hat{\beta}\|_2 \le \|\hat J-J^*\|_F/\lambda$. It is therefore desirable that $\lambda$ be large.

A simple setting where this holds is when the $J_i$'s are orthogonal with respect to the trace inner product, namely, $\mathrm{trace}(J_i^\top J_j) = 0$ for $i\ne j$. In this case, $\lambda = \min_i \|J_i\|_F$, and if all matrices have $\|J_i\|_F\ge \Omega(\sqrt{n})$ then the rate is $|\hat\beta-\beta^*|\le \sqrt{k\log n/n}$.\footnote{Notice that $\|J_i\|_F$ is always upper bounded by $O(\sqrt{n})$ if $\|J_i\|_\infty = O(1)$.}
Note that orthogonality holds when the matrices have a disjoint support. For an example, assume that each $x_i$ represents a person which resides in one of $\ell$ countries and $k = \ell + \binom{\ell}{2}$: each $J_i$ either represents the connections within a specific country or connections between people across two specific countries. The matrices $J_i$ have disjoint support, hence they are orthogonal. For another  example of disjoint supports, assume that we are taking snapshots of a network $(V,E)$ across $T$ different time steps, where $n = |V|T$ and $x_{v,t}$ corresponds to the snapshot of node $v\in V$ at time $t \in [T]$. We have two interaction matrices, $J_1$ which corresponds to temporal interactions: $(J_1)_{(v,t),(u,s)} = \mathbf{1}(u=v \wedge |t-s|=1)$ and $J_2$ which corresponds to spatial interactions: $(J_2)_{(v,t),(u,s)} = \mathbf{1}((u,v)\in E \wedge t=s)$. These matrices clearly have disjoint supports. 

For an example where estimation of ${\beta}$ is possible without orthogonality, suppose that each $J_i$ is the incidence matrix of a graph $([n], E_i)$, and define $\lambda_i = |E_i \setminus (\bigcup_{j \in [n]\setminus\{i\}} E_j)|$,
namely, $\lambda_i$ is the number of connections unique to network $i$. Then, Theorem~\ref{thm:informal-main} guarantees
\begin{equation} \label{eq:553}
\sqrt{\sum_i \lambda_i(\hat{\beta}_i - \beta^*_i)^2} \le \sqrt{k \log n}; \quad \text{ and } \|\hat{{\beta}}-\beta^*\|_2 \le \sqrt{k\log n/\min_i\lambda_i},
\end{equation}
Hence, we can accurately learn the parameters of networks with many unique connections.

==> intro_old.tex <==
\newpage
\setcounter{page}{1}

\section{Introduction}

%\yuval{Current structure: (most parts should be shortened)\\
%Motivation and problem definition, first 3 pages \\
%Dobrushin's condition \\
%Results \\
%Prior work (should be revised) \\
%Techniques
%}

%\yuval{Meetings' comments:
%Convince that we are overcoming technical challenges.\\
%}

%----------------- PROSE ----------------------
% stats from dependent data motivation

Loosely defined, statistical inference is the task of using multiple observations of some probabilistic phenomenon to estimate aspects of that phenomenon that are of interest and can be identified from the available data. An important setting that has seen much progress is that wherein the observations can be modeled as independent samples from a probability distribution that we are seeking to learn, in some way.
%Statistics involves collecting data in various forms from a myriad number of sources to perform inference and prediction tasks. When analyzing the procedures we employ to draw conclusions from this data, a common assumption made is that of independence between samples. 
However, rarely does this independence assumption hold. Observations collected on a spatial domain, temporal domain or social network are commonly intricately dependent. Rather than  viewing it as a set of $n$ independent samples, in these settings it is more fitting to view the data as a {\em single} sample from an $n$-dimensional distribution. {\em What can be inferred for that $n$-dimensional distribution from a single sample?} 

The ubiquity of data dependencies in the natural world, as well as in social, financial and networked environments has motivated the development of statistical inference frameworks, which both model and seek statistical guarantees under data dependencies. This pursuit has a long history in Statistical Physics, Probability Theory, Econometrics, and Machine Learning, and has recently been studied in the Theory of Computation---see e.g.~\cite{besag1974spatial,yu1994rates,chatterjee2007estimation,kontorovich2008concentration,berti2009rate,mohri2009rademacher,pestov2010predictive,mohri2010stability,kuznetsov2015learning,McDonald2017,kontorovich2017concentration,bhattacharya2018inference,ghosal2018joint,bresler2018optimal,daskalakis2019regression,dagan2019learning,valiant2019worstcase}. Our goal is to advance the algorithmic and probabilistic foundations of this important and emerging field.



%Dependence amongst samples can arise in a number of ways and in many scenarios the dependence is significant. In these scenarios, rather than viewing the data as a set of $n$ independent samples, it must be viewed as a single sample from a $n$-dimensional distribution. In this work, we explore how we can perform inference in a certain correlation model which uses such high-dimensional distributions with a succinct description. Our model will be well-suited to modeling many correlation scenarios. One particular scenario which we focus on as a running example is when the data collected from a social network. As a motivating example, consider the following situation: we observe whether people buy an \emph{iPhone} or an \emph{Android phone} along with their underlying social network (such as Facebook) and we wish to understand the strength of the network effects on any individual's decision. 
%\yuval{Is this a good example? After Cambridge analytica, will people want to support such a paper? DELETE COMMENT BEFORE WE UPLOAD!!!!!!}

% inference in Ising models motivation

\medskip We will focus our attention on the celebrated {\em Ising model}~\cite{ising1925beitrag}, a canonical Markov Random Field with pairwise interactions, which samples a binary vector $x = (x_1,\ldots,x_n) \in \{\pm 1 \}^n$, according to the  measure:
\begin{align}
\label{eq:ising}
    \Pr_{J^*}[x] = \exp\left(x^{\top}J^*x/2 - F(J^*) - n\log 2 \right);~\text{where}~ 
    F(J^*) = \log \left( 2^{-n}\sum_{x \in \{\pm 1 \}^n} \exp(x^{\top}J^*x/2 )\right).
\end{align}
Here, $J^*$ is an $n \times n$ symmetric matrix with zero diagonal and $F$ is the so-called log-partition function. Notice that the term $J^*_{ij} x_i x_j$ in the exponent of the density encourages $x_i$ and $x_j$ to have equal or opposite signs depending on the sign and magnitude of $J^*_{ij}$, but this ``local encouragement'' can be overwritten by indirect interactions arising through paths between $i$ and $j$ in the graph defined by $J^*$. Whenever $i$ and $j$ are disconnected in this graph, $x_i$ and $x_j$ are independent.

 The Ising model has found many applications in a range of disciplines, including Statistical Physics, Computer Vision, Computational Biology, and the Social Sciences~\cite{GemanG86,Ellison93,Felsenstein04,chatterjee2005concentration,DaskalakisMR11,daskalakis2017concentration}. For example, it has been used to model binary behavior on a social network~\cite{Ellison93,young2006diffusion,montanari2010spread}, wherein nodes choose between, say, whether to own an Android phone ($+1$) or an iPhone ($-1$), and $\sum_j J^*_{ij}x_ix_j$ captures the utility derived by node $i$ depending on her and the other nodes' selection of phones. In this setting, it is easy to show that, when nodes update their strategies using logit best response dynamics, the stationary distribution of their joint behavior converges to~\eqref{eq:ising}.
 
 Given its broad applicability, a long line of research has aimed at estimating Ising models from samples. For some exciting progress on this front in recent years, see e.g.~\cite{santhanam2012information,ravikumar2010high,bresler2015efficiently,vuffray2016interaction,klivans2017learning,hamilton2017information,wu2019sparse}. Importantly, these works assume access to {\em multiple samples} from the Ising model, and target estimating the interaction matrix $J^*$, under some conditions. {\em Instead our focus in this work will be to estimate $J^*$ from a {\em single} sample}. This is well-motivated in many  applications of the model where we can realistically only collect a single sample from the distribution. In our earlier example, we can take a snapshot of the network to see who is using an Android phone or an iPhone. If we take a snapshot of the network tomorrow, chances are that very little would have changed, and we certainly would not collect an independent sample from the model. Such lack of access to independent samples is ubiquitous in financial, meteorological, and geographical data, as well as social-network data~\cite{manski1993identification,bramoulle2009identification}, and has been studied in topics as diverse as criminal activity (see e.g. \cite{glaeser1996crime}), welfare participation
(see e.g. \cite{bertrand2000network}), school achievement (see e.g. \cite{sacerdote2001peer}), participation in
retirement plans~\cite{duflo2003role}, and obesity~\cite{christakis2013social,trogdon2008peer}.

\medskip Estimating the parameters of Ising models from a single sample has recently seen some important advances. As $J^*$ has $O(n^2)$ parameters, it is clear that some restriction must be placed on it for it to be estimable at all from a single observation. One well-studied assumption is that $J^*=\beta J$, where $J$ is a known matrix, and $\beta$ is an unknown scalar strength parameter, i.e.~that the interaction strenghts are all known up to a scalar multiple. In this setting, \citet{chatterjee2007estimation} has shown that $\beta$ can be estimated to within $O(1/\sqrt{n})$ whenever the log-partition function of the model satisfies $F(J^*) \ge \Omega(n)$, and follow-up work has been able to generalize his result to broader settings~\cite{bhattacharya2018inference,ghosal2018joint,daskalakis2019regression}.
 
%starting point in our approach is the Ising model~\cite{ising1925beitrag}, which is a popular model with roots in statistical physics which captures dependence between different samples using pairwise interactions between them (pairwise interactions can lead to long-range interactions as well). It is a canonical example of an undirected graphical model with a rich literature and applications in a wide range of fields \cite{?,?,?}. 

%Below, we state the model in its simplest form which already allows us to model interesting correlation effects. Each variable $x_i$ in the Ising model takes values in $\Omega = \{\pm 1 \}$ and the joint distribution over $x = (x_1,\ldots,x_n)$ is given by
%\begin{equation}
%\label{eq:ising}
%    \Pr[x] = \exp\left(x^{\top}J^*x/2 - F_n(J^*) - n\log 2 \right); \quad \text{ where } 
 %   F_n(J^*) = \log \left( 2^{-n}\sum_{x \in \{\pm 1 \}^n} \exp\left(x^{\top}J^*x/2 \right) \right)
%\end{equation}
%where $J^*$ is an $n \times n$ symmetric matrix with zeros on the diagonal and $F_n$ is known as the log-partition function of the model. \yuval{changed $\beta x^\top J^* x$ into $x^\top J^* x$. This way, the above equation is compatible with our model as well ....TBC}
%\yuval{Added normalization to $F_n$ to be consistent with prior work (we need to compare later)}


%It is common to write $J^* = \beta^* J$, where $J$ is some base matrix and $\beta^* \in \mathbb{R}$ is a parameter that signifies the strength of the network effects on the graph defined by the matrix $J$. 
%The Ising model is a powerful tool to model correlated samples. We present an example from social network analysis where the model comes in handy.
%Consider a social network defined by a graph $G = (V,E)$ where each individual chooses one of two options (for instance an iPhone vs an Android phone). A stochastic process over $G$ ensues wherein in each time step, a person is randomly chosen and her/his choice is updated according to the choices her/his peers have at that stage with some noise added to it. \cite{montanari2010spread} show that this process eventually converges to the Ising model. They use this model to study how new innovations spread in a social network.
%\yuval{commented out the second example since it assumes external field and to save space}
%\item Consider a setting where we are doing logistic regression on $n$ people on a social network. The choice $y_i \in \{\pm 1 \}$ made by each individual depends on their intrinsic features $x_i$ and also upon the choices made by their peers $y_j, j \in N(i)$ ($N(i)$ denotes the set of neighbors of $i$). The joint distribution on the set of $\{y_i\}_{i=1}^n$ can be represented using an Ising model (with the addition of a linear term inside the $\exp(.)$ known as the external field of the model) \cite{daskalakis2019regression}.\yuval{Perhaps modify a bit? We don't do an external field here, so it' better to have a motivated example for our model.}
%Apart from the above, the model has found applications in computer vision \cite{?}, neuroscience \cite{?}, phylogenetics \cite{?} among others.\\

%Consequently, inference of the parameters of different formulations of an Ising model from samples is an important and well-studied problem.  
%In particular for the formulation \eqref{eq:ising}, inferring the parameter $\beta^*$ from a \emph{single} sample of the Ising model is studied in the works of \cite{chatterjee2007estimation,bhattacharya2018inference,ghosal2018joint,daskalakis2019regression}.

However, the afore-described assumption about $J^*$ is only a first step towards modeling more realistic scenarios. In practice, it might be an unreasonably strong assumption that the interaction strengths are known up to some scalar multiple. Indeed, nodes commonly belong to several networks which might contribute to their behavior at different degrees of importance. To capture such settings, we study the case that $J^*$ is an unknown linear combination of $k$ known community matrices, yielding the model
\begin{align} \label{eq:ourmodel}
    \Pr_{J^*}[x] = \exp\left(x^{\top}J^*x/2 - F(J^*) - n\log 2 \right); \quad \text{where } J^* = \sum_{i=1}^k \beta_i J_i.
\end{align}
Here, $\{ J_i \}_{i=1}^k$ are community matrices, each symmetric with zeros on the diagonal, $\beta=\{\beta_i\}_{i=1}^k$ are scalar parameters signifying the varying importance of each community, and $F(J^*)$ is as defined in \eqref{eq:ising}. Our goal is to estimate $J^*$ given $\{ J_i \}_{i=1}^k$ and one sample $x \sim \Pr_{J^*}$, namely

\vspace{5pt}\framebox{\begin{minipage}[h]{15.3cm} {\em Single Sample Inference of an Ising Model with Multiple Parameters:} {Given a collection of community matrices $\{ J_i \}_{i=1}^k$ as well as a single sample $\{\pm 1\}^n \ni x$ from \eqref{eq:ourmodel}, compute an estimate $\hat{J}(x)$ to minimize $\|\hat{J}(x)-J^* \|_F$.}
\end{minipage}
}



%Our problem has many interesting applications. In our earlier example, nodes might belong to multiple communities $J_1,\ldots,J_k$, and each community might contribute to the choice of phone technology at different strength.
\medskip A few remarks are in order. First, model~\eqref{eq:ourmodel} adds a lot of expressive power to the single-parameter setting ($k=1$) studied in earlier work. For example, we might have access to various social networks that individuals belong to (Facebook, LinkedIn, etc.) and expect that they all contribute to their behavior at different strengths. As another example, we might not know the interaction matrix, but might be comfortable postulating that it comes from some parametric family  of matrices, and we might be seeking to estimate it. This is a common challenge in Spatial Econometrics~\cite{anselin2001spatial,lesage2008introduction,anselin2012new,anselin2013spatial}. As a final example, we  might be studying the temporal evolution of a network, such as the voting pattern within a district over a number of election cycles. A reasonable modeling assumption is that a person's vote in any particular cycle correlates with the votes of his peers in that cycle and also his vote in the past cycle. However the strength of the spatial correlation (with peers) might be different from that of the temporal correlation (with past vote).

%\begin{enumerate}
%    \item Suppose we have access to multiple networks (Facebook, Linkedin, etc.) with different interaction strengths and all the networks influence an individual's decision. Our model captures this setting.
 %   \item Suppose that the interaction strength is according to some distance metric that is not known, however, we know that it is one of the candidates $\{J_1,J_2,\ldots,J_k\}$. Our model can be used this setting as well.
  %  \item Geographical Econometrics reference and explanation.
   % \item Suppose we are studying the temporal evolution of a network. For instance, we record the voting pattern within a district over a number of election cycles. A reasonable modeling assumption is that a person's vote in any particular cycle correlates with the votes of his peers in that cycle and also his vote in the past cycle. However the strength of the spatial correlation (with peers) might be different from that of the temporal correlation (with past vote).
%\end{enumerate}



%$J^*$ lies in a $k$-dimensional subspace $V$ of the space of $n\times n$ matrices, 
%\yuval{Modified a bit, to define the communities as non-orthogonal. In fact, we don't have to talk of an orthogonal basis at any point. Deferring the definition of $V$ a bit.}



% The joint distribution of $x$ is then given by
% \begin{equation}
% \label{eq:ourmodel}
%     \Pr[x] = \exp(x^\top J^* x) / Z_{J^*} ; \quad
% Z_{J^*} = \sum_{x \in Q_n} \exp(x^\top J^* x).
% \end{equation}







% present formal problem definition in a box here
%\yuval{why do we need to define it here? Haven't we defined it above already?}
%\nishanth{I think it would be good to have the formal problem specification that is easy to spot at some point around here?\\}

Our second remark is to point out that we have formulated our problem as that of estimating $J^*$ rather than estimating the parameters $\beta_1,\ldots,\beta_k$. This choice is necessary to make our problem statistically meaningful and feasible. Indeed, if the matrices $J_1,\dots,J_k$ are (close to being) linearly dependent, then there is no hope in targeting an estimation of the parameters $\beta_1,\dots,\beta_k$. Hence, we focus on learning the linear combination $\sum_i \beta_i J_i$ to high accuracy, where the error is measured according to the Frobenius norm, and this metric captures our learning capacity exactly in many cases, as we discuss below. In some applications, estimates of $\beta_1,\ldots,\beta_k$ can be directly obtained from an estimate of $\sum_i \beta_i J_i$. This is common when  $J^*$ belongs to some parametric family of interaction matrices, or when the constituent $J_i$'s have structure, as we discuss below.

%We note that in some applications it may be more suitable to optimize for the parameters directly and this is left for future work. We discuss what assumptions on $J^*$ are needed to make the problem statistically meaningful and feasible. First of all, n

Finally, we need to assume a bound on the interaction strengths in $J^*$, otherwise we could observe nearly deterministic behavior, with different values of $J^*$ leading to indistinguishable distributions.\footnote{This is due to the flattening behavior of the sigmoid function when its argument is a large value.} We will make the common assumption that $\|J^*\|_\infty := \max_{i \in [n]} \sum_{j \ne i} |J^*_{ij}| \le M$, where $M$ can be any \emph{constant}.\footnote{When this assumption is violated, it might become information-theoretically impossible to have a consistent estimator for $\beta$.} This models settings where no node has an overwhelming influence on the other nodes. It is important to note that a constant bound on $M$ is different from saying that the model satisfies the more stringent Dobrushin condition.\footnote{Dobrushin's uniqueness condition, discussed in Section~\ref{sec:technical-lemmas} and formally in Appendix~\ref{sec:dobrushin}, is a well-studied condition in Statistical Physics under which the correlations among variables are relatively weak. Ising models with $\|J^*\|_\infty < 1$ satisfy this condition.} Indeed, a constant upper bound on $M$ allows models that that do not satisfy Dobrushin's condition and that are in {\em low} temperature.
%\yuval{Shouldn't we say what is Dobrushin's condition.} \costis{Sure, there is a footnote later about Dobrushin which can be moved here. By the way, the discussion about Dobrushin in section 1.3.1 is not entirely accurate right? As in, is Dobrushin's stated w.r.t. the infinity norm of the J matrix or in terms of sum of influences in terms of TV distances of different conditional distributions or in some other way?}\yuval{Yeh, I made a small modification to fix that.}

%\yuval{Commented out most of the discussion.}
%\begin{itemize}
    % \item \yuval{Removed the discussion of small entries, as it is clear that this is impossible. On the other hand, the infinity norm assumption does require elaboration.} If the matrices $\{J_1,\dots,J_k\}$ are close to being linearly dependent, then we will not be able to distinguish between different values of $\vec{\beta}$. Hence, instead, our goal would be to learn a matrix $\hat{J}$ which is close to $J^*$ with respect to some matrix distance. We selected to minimize $\|\hat{J}-J^*\|_F$, where $\|A\|_F^2 := \sum_{i,j} A_{ij}^2$ is the Frobenius norm. This guarantees that we can learn learn the parameters that stand out, namely those that cannot be represented as a linear combination of the other parameters, and furthermore, learn most of the pairwise correlations. In addition, we found it to be very suitable mathematically, since the optimal estimation rate (error) has a simple form in a large regime of the parameters. Still, for some applications a different a different metric may be a better fit, and this is left for future work.
    %\item If the entries of $J^*$ are too large, then again different values of $\vec{\beta}$ lead to indistinguishable distributions\footnote{This is due to the flattening behavior of the sigmoid function when its argument is a large value.}. Quantitatively, we will take the common assumption that $\|J^*\|_\infty := \max_{i \in [n]} \sum_{j \ne i} |J^*_{ij}| \le M$, for some parameter $M>0$ which is a constant\footnote{when this assumption is violated it might become information-theoretically impossible to have a consistent estimator for $\beta$.}. This assumption is similar to the bounded \emph{width} assumption in the work of \cite{klivans2017learning} and allows for bounded degree graphs and dense graphs (with the average edge strength decreasing as the degree of a node grows). It models the situation where no node has an overwhelming influence on its environment and results in a clean model that is simpler to analyze. Some of the prior works assume spectral norm boundedness $\| J^* \|_2 \le M$ \cite{chatterjee2007estimation,bhattacharya2018inference} which is a slightly weaker assumption.
%\end{itemize}
%\begin{itemize}
%    \item Multiple social networks.
%    \item Geographical Network Data
%\end{itemize}


\paragraph{Section organization.}
We present our main results in Section~\ref{sec:intro-results}, starting with our theorem for general values of $k$, which generalizes prior work, and proceeding with our result for $k=1$, which improves over prior work. We also present an impossibility result, establishing that our main result for $k>1$ is tight. Additionally, we provide a detailed comparison of our work to the existing literature. In Section~\ref{sec:technique}, we highlight some new techniques used in our proofs, which may have applications outside the scope of this paper, followed by a proof sketch of our main results. We postpone the full details of our paper to Sections~\ref{sec:pr-multiparam}---\ref{s:lower_bound}.

==> old.tex <==
\section{Old stuff}
\subsection{Intro}
We would like to learn an Ising model from samples. In particular, assume a distribution over $x \in Q_n:= \{-1,1\}^n$ such that
\[
\Pr[x] = \exp(x^\top A^* x) / Z ; \quad
Z = \sum_{x \in Q_n} \exp(x^\top A^* x).
\]
We will assume that $A^*$ lies in some $k$-dimensional subspace $V$ of the space of $n\times n$ real matrices, containing only symmetric matrices with zeros on the diagonal. Additionally, assume that $\|A^*\|_\infty := \max_{i \in [n]} \sum_{j \ne i} |A^*_{ij}| \le M$, for some parameter $M>0$ which is usually considered to be a constant. Let $B_{\infty,M}$ denote the set of all matrices with an infinity norm of at most $M$.

We don't know $A^*$, and we just get one sample $x\sim \Pr_{A^*}$ and our goal is to estimate it. We will compute the maximum pseudo likelihood:
\[
\arg\max_{A \in V \cap B_{\infty,M}} PL(A ; x) := \arg\max_{A \in V \cap B_{\infty,M}} \prod_{i\in [n]} \Pr_A[x_i | x_{-i}].
\]
Denote the maximizer by $\hat{A}$ (if there are multiple maximizers, we will select one of them arbitrarily).

**** Make the orthogonal basis be $A^{(i)}$ rather than $A_i$.

We would like to estimate the quality of $\hat{A}$, in particular, we would like to minimize $\|\hat{A}-A^*\|_F$, namely, the Frobenius norm of this difference. For this purpose, we will calculate the negative log likelihood of each $A$, then the derivatives and second derivatives. Let's parameterize each $A\in V$ by a vector $\beta \in \mathbb{R}^k$: assume that $A_1, \dots, A_k$ is an orthonormal basis for $V$, namely, $\|A_i\|_F = 1$ for all $i \in [k]$ and $tr(A_i^\top A_j) = 0$ for all $i \ne j$. For any $\beta \in \mathbb{R}^k$, denote $A_\beta = \sum_i \beta_i A_i$, and note that $\beta \mapsto A_\beta$ is a unitary bijection from $\mathbb{R}^k$ to $V$, namely, $\|A_\beta\|_F = \|\beta\|_2$ for all $\beta \in \mathbb{R}^k$. We will write the log likelihood in terms of $\beta$: first, let $\varphi(\beta) = - \log PL(A_\beta;x)$. Given $\beta \in \mathbb{R}^k$ and $i \in [n]$, define $m_{\beta,i}(x) = (A^\beta x)_i$. For a function $g \colon \mathbb{R}^k \to \mathbb{R}$ and $v \in \mathbb{R}^k$, define $\partial g/\partial v = v^\top \nabla g$, as usual. Then, notice that
\begin{align}
\varphi(\beta) &= \sum_{i=1}^n \log\cosh(m_{i,\beta}(x)) - x_i m_{i,\beta}(x) + \log 2 \\
\frac{\partial \varphi(\beta)}{\partial v}
&= \sum_{i=1}^n 
m_{v,i}(x) (\tanh(m_{\beta,i}(x))-x_i) \\
\frac{\partial^2 \varphi(\beta)}{\partial v^2}
&= \sum_{i=1}^n
m_{v,i}(x)^2 \sech^2(m_{\beta,i}(x)).
\end{align}

Let $B$ denote the set of all values of $\beta$ such that $\|A_\beta\|_\infty \le M$. Then, our estimation task boils down to finding 
\[
\hat\beta
= \argmin_{\beta \in B} \varphi(\beta).
\]

\subsection{Concentration inequality multivariate}

This is a part of a more general theorem (Do only if we have enough time..). There, we have some discrete $k$-th order derivative $\tilde D^{(k)}$ of dimensions $n_1, \dots, n_k$. An $k+1$th order derivative is a function $\tilde D^{(k+1)} \colon \{-1,1\}^n \to \mathbb{R}^{n_1\times\cdots \times n_{k+1}}$ that satisfies: for any vectors $u^{(i)} \in \mathbb{R}^{n_i}$ ($i \in [k]$) and for any $x$, we have
\[
\sum_{i_{k+1} \in [n_{k+1}]}\left(\sum_{i_1\in [n_1], \dots, i_k \in [n_k]} \tilde D^{(k+1)}(x) \prod_{j \in [k]} u^{(j)}_{i_j}\right)^2
\ge \|D\left(\sum_{i_1\in [n_1], \dots, i_k \in [n_k]} \tilde D^{(k)}(x) \prod_{j \in [k]} u^{(j)}_{i_j} \right)\|_2
\]
*** Define the tensor product properly.


\subsection{Sparse learning with multiple parameters}

*** Issue: the derivative may be large, also for parameters that correspond to the orthogonal subspace $M^\perp$. ***

Assume that we have $\ell$ parameters but the model is $k$ sparse. Say, we use the $\ell_1$ norm. There are some issues so we cannot use exactly the technique as a black box:
\begin{itemize}
	\item First, the derivative is not known ahead, and it can be affected by the strong convexity parameter.
	\item Secondly, we are not necessarily strongly convex in the true subspace. 
\end{itemize}
See if those issues matter. In fact, we can use the fact that the strong convexity parameter does not change much throughout the program. Hence, even if the derivative is large, the strong convexity will be large and we'll get rid of it pretty quickly. 
For the second issue: although we're not necessarily strongly convex, this shouldn't matter probably. Namely, if we move around the non-strongly convex direction, the other derivatives shouldn't change much. 

\begin{itemize}
	\item Can we find a better regularization?
	\item Even if the derivative is large in the true parameter, we can possibly find a different point that lies in the same subspace and close to the true parameter where the derivative is small. Use this point as a "pivot": assume that the new point is actually the true parameter, and there the derivative is low, so we can show that the true parameter is actually not far from this point. By triangle inequality, it will be close to the original parameter.
	\item Perhaps assume that within the subspace of true parameters, we are strongly convex: namely, the matrices corresponding to the true parameters are sufficiently far. If not, we can find a subset of these containing most of the mass, such that we are, indeed, strongly convex in their span, and use the theorem for the non-realizable setting.
\end{itemize}


the parameters that constitute the network are 

... efficient algorithms

\subsection{General concentration inequalities}

Not sure if this is useful..

The following results assume that the independence matrix $A$ of $x$, satisfies $\|A\|_\infty \le M$ where $M$ is a constant. We have the following bounds.
Anti-concentration of linear functions:
\begin{lemma}
	Assume that for each $x$ we have that for any $i$ and any $x_{-i}$, $\Var(x|X_{-i}=x_{-i}) \ge \gamma$. Let $a_1,\dots, a_n \in \mathbb{R}$. Then,
	\[
	\Var(\sum_i a_i x_i) \ge f(M,\gamma) \sum_i a_i^2,
	\]
	where $f$ is some function.
\end{lemma}
Next, we have concentration of functions, by adapting the proof of the "note". (see above) This is in fact for Dobrushin's condition.

Next, a concentration of conditionally zero functions:
\begin{lemma}
	Let $f_1,\dots, f_n$ be some functions. Then, for any $p$,
	\[
	\|\sum_i f_i(x) \|_p^p
	\le f(M) \max_{I,x_{-I}, \alpha_i} \E[(\sum_{i \in I} \alpha_i f_i(x))^p|x_{-I}]
	\]
	where the maximum is over all sets $I$ such that $\|A_I\|_\infty \le 0.1$ (where we take by $\alpha_I$ the set of corresponding rows and columns of $I$) and $1\le \alpha_i\le 2$. (probably $\alpha_i$ can be removed)
\end{lemma}
In the above lemma it would be particularly convenient to assume for any $i$ and $x_{-i}$, $\E[f_i(x)|x_{-i}] = 0$.

From the anti-concentration for linear functions, we get that for a PSD polynomial $x^\top A x$, $\E[x^\top A x] \ge C tr(A)$. However, we can also get high concentration:
Lastly, we have a lemma for 2nd degree polynomials:
\begin{lemma}
	Let $A$ be a PSD matrix, and $x$ has a minimal conditional probability of $\gamma'$, namely, given $x_{-i}$, each value of $x_i$ is obtained with probability at least $\gamma'$, and also, conditional variance of at least $\gamma$ (as defined above). Then,
	\[
	\Pr[x^\top A x \le f(\gamma',\gamma,M) tr(A)] \le e^{-c tr(A)/\|A\|_2}.
	\]
	(if I'm not wrong)
\end{lemma}


\subsection{Lower bound}

We want to show that $\sqrt{k}$ is also a lower bound on the rate. We start with the following lemma:
\begin{lemma}
	Let $P$ and $Q$ be two distributions on $\{-1,1\}^n$ corresponding to Ising models with interaction matrices $A$ and $B$, and zero external field, such that $\|A\|_2, \|B\|_2 \le 1 - \Omega(1)$. Then,
	\[
	TV(P,Q) \le C \|A-B\|_F^2 \log n.
	\]
\end{lemma}
\begin{proof}
	Proof is completely wrong.
	\if 0
	Let $k = O(n \log n)$, and we will create a greedy coupling between the Glauber dynamics with respect to both $P$ and $Q$, for $k$ step. Let $X_0, X_1, \dots, X_k$ denote an execution of the Glauber dynamics with respect to $P$, where $X_0 \sim P$ and $X_t$ is obtained from $X_{t-1}$ by applying one step of the Glauber dynamics according to $P$. Let $Y_0, \dots, Y_k$ be defined such that $Y_0 \sim P$, and $Y_t$ is obtained from $Y_{t-1}$ according to the Glauber dynamics with respect to $Q$. We will couple $Y_t$ and $X_t$ such that $Y_0 = X_0$, and for $t \ge 1$, $X_t$ and $Y_t$ are obtained from $X_{t-1}$ and $Y_{t-1}$ according to the greedy coupling. Namely, the same coordinate is re-sampled, and it is sampled to be the same with probability the highest probability possible.
	
	Now, let $E_{t,i}$ denote the event that $t$ is the first time where $X_t$ and $Y_t$ differ and coordinate $i$ is changed at time $t$. We will show that with constant probability, none of the events $E_{t,i}$ hold. This will imply that $X_k = Y_k$ with constant probability. Let $T_{t-1,i}$ denote the total variation between the conditional distribution of $X_{t-1,i}$ conditioned on $X_{t-1,-i}$, and the conditional distribution of $Y_{t-1,i}$ conditioned on $Y_{t-1,-i}$, and let $I_t$ denote the coordinate changed at time $t$. Then,
	\[
	\Pr[E_{t,i}|X_{t-1},Y_{t-1}] = T_{t-1,i} \mathbf{1}(X_{t-1}\ne Y_{t-1})\Pr[I_t=i]  = T_{t-1,i}\mathbf{1}(X_{t-1}\ne Y_{t-1})/n.
	\]
	Next, notice that 
	\[
	T_{t-1,i} = |\tanh((A X_{t-1})_i) - \tanh((B Y_{t-1})_i)|/2
	\le |A_i^\top X_{t-1} - B_i^\top Y_{t-1}|/2,
	\]
	using the fact that $\tanh$ is $1$-Lipschitz. Therefore,
	\[
	T_{t-1,i}\mathbf{1}(X_{t-1}\ne Y_{t-1})
	\le |(A_i - B_i)^\top X_{t-1}|.
	\]
	\fi
\end{proof}

\section{Technique}


Should probably contain the following:
\begin{itemize}
	\item Discussion of prior techniques.
	\item Why they don't work.
\end{itemize}

Elaborate:
\begin{itemize}
	\item Relative fluctuation of derivatives
	\item For the derivative: we condition and then apply concentration results. The others don't condition,
	they use exchangeable pairs so they obtain absolute bounds. 
	Moreover, they don't use as strong concentration as
	we do.used Chatterjee's exchangeable pair.
	\item (1) arguments specific for one matrix parameter using the structure of the log partition function, (2) Nishanth: argument that holds only when $\|J\|_F$ is $\Omega(\sqrt{n})$. -> Variance argument is new.\\
	Use of the improved concentration inequality
	along with the conditioning to obtain high probability anticoncentration bounds that match the lower bounds (variance bound could still be derived using prior techniques)
	\item Recent result for concentration for polynomials for second derivative.
	\item Multiple parameters: high probability bound and then union bound (not used in the prior one-sample papers). Others have one parameter so they don't need a high probability bound.
\end{itemize}

\subsubsection{Applications of the technique.}
\begin{itemize}
	\item Conditioning can be applied under the more general Dobrushin's condition.
	\item For general PMLE: as $\varphi'$ will typically be zero.
	\item To prove inequalities previously proven by the exchangeable pair technique.
\end{itemize}

\subsubsection{Old comparison}
\yuval{Should probably be significantly shortened.}
\begin{itemize}
	\item 
	All prior work \cite{chatterjee2007estimation,bhattacharya2018inference,ghosal2018joint,daskalakis2019regression} bounded the first and second derivatives of the PMLE separately, rather than bounding the ratio between them (see Section~\ref{sec:conditioning}). To achieve the desired bounds, they relied on regularity assumptions, either assuming that the partition function is of maximal order \cite{chatterjee2007estimation}, that it is of the same order in a neighborhood of $\beta^*$ \cite{bhattacharya2018inference}, or a lower bound on the Frobenius norm \cite{ghosal2018joint,daskalakis2019regression}, assumptions that we remove.\footnote{\citet{ghosal2018joint}, in fact, assumes a lower bound in a different quantity that corresponds to the setting studied in their paper. This assumption is implied by a Frobenius norm bound.}
	\item A lower bound on the second derivative ($x^\top J^\top J x$) for one parameter estimation: prior work~\cite{chatterjee2007estimation,bhattacharya2018inference} relies on the idea that the partition function is defined in terms of $\sum_\sigma \exp(\beta^* x^\top J x)$ to show that $x^\top Jx$ is large with high probability whenever the partition function is large. Then, they argue that $|x^\top J^\top J x - xJx|$ is small, as this quantity corresponds to the derivative of the PMLE. Hence, $x^\top J^\top J x$, which corresponds to the second derivative, has nearly the same magnitude as $xJx$, therefore it is lower bounded.\footnote{Notice that the bound on the derivative is used in the bound on the strong convexity. However, it is just used in order to show that $x^\top J x$ and $x^\top J^\top Jx$ are of the same order, and the lower bound on $x^\top J x$ is independent of the upper bound on the derivative.}
	\item Hessian lower bound for one matrix parameter and linear parameters: Notice that the technique from the previous bullet would only succeed in bounding the polynomial $x^\top J^\top Jx$, hence not generalize to multiple parameters. To tackle this problem, \cite{ghosal2018joint} suggested a reduction to the Curie Weiss model which is specific for learning one linear parameter and \cite{daskalakis2019regression} suggested an indexing technique based on Chatterjee's exchangeable pairs that required many entries of $J$ to be large.
	\item Multiple matrix parameters: in this scenario, the partial derivatives can be of the form $x^\top J_{\vec{\beta}}^\top J_{\vec{\beta}} x$, where $J_{\vec{\beta}}$ is an arbitrary linear combination of the parameter matrices $J_i$. It is likely that \emph{there exists} some $J_{\vec{\beta}}$ that will not satisfy the regularity assumptions from prior work, and the proof would not go through. Hence, we instead provide general lower bounds on second degree polynomials (\ref{sec:conditioning}). Furthermore, when many parameters are involved, the determinant of the Hessian used in \cite{daskalakis2019regression,ghosal2018joint} does not capture well its minimal singular value.\footnote{\cite{daskalakis2019regression} resolved this issue by assuming that the linear parameters are fixed and already }. Instead, we derive high probability bounds lower for each specific polynomials, that follow from the conditioning technique (Lemma~\ref{lem:informal-subsample}), then deriving the result by a union bound on exponentially many partial derivatives.
\end{itemize}

\subsubsection{Older}
Below, we outline the proof idea and techniques, starting with an estimation of one parameter.
The standard approach of \emph{Maximum likelihood estimation} (MLE), that outputs $\widehat{\beta}$ which maximizes the probability of drawing the obtained sample $x$, namely, $\widehat{\beta} := \argmax_{\beta} \Pr_{\beta}[x]$. 
%where $x$ is the sample from the distribution $\Pr_{\beta^*}$ parametrized by an unknown $\beta^*$, and $\Pr_{\beta}[x]$ is the probability of $\beta$ to draw $x$. 
While the MLE requires computing the partition function which is NP hard to approximate, a recourse is to optimize the \emph{pseudo MLE} (PMLE) of \cite{besag1974spatial,besag1975statistical} instead: $\argmax_{\beta}\prod_{i = 1}^n \Pr_{\beta}[x_i \mid x_{-i}]$, where $\Pr_{\beta}[x_i\mid x_{-i}]$ is the probability of $\Pr_{\beta}$ to draw $x_i$ conditioned on the remaining entries of $x$, denoted $x_{-i}$. One typically minimizes the negative log PMLE,
\begin{equation} \label{eq:varphi}
\varphi(x;\beta)
:= \argmin_{\beta} -\sum_{i=1}^n \log\Pr[x_i \mid x_{-i};\beta],
\end{equation}
which is a convex function in the parameters $\beta$ whose global optima can be subsequently found using an appropriate first-order optimization technique. The error $|\beta^*-\hat{\beta}|$ is approximated by $\varphi'(x;\beta^*)/\varphi''(x;\beta^*)$, where $\varphi'$ and $\varphi''$ are the first and second derivatives of $\varphi$ with respect to $\beta$ and we are assuming that $\partial''$ does not significantly change in a neighborhood of $\beta^*$. The main challenge, faced also in prior work \cite{chatterjee2007estimation,bhattacharya2018inference,ghosal2018joint,daskalakis2019regression}, is to bound this ratio.

Notice that $\varphi'(\beta^*;x)$ and $\varphi''(\beta;x)$ are functions of $x=(x_1,\dots,x_n)$. There are a variety of concentration inequalities for \emph{independent} random variables $f(x_1,\dots,x_n)$ \cite{boucheron2013concentration} and many of them were generalized for weakly correlated variables under Dobrushin's condition \cite{kulske2003concentration,chatterjee2005concentration,daskalakis2017concentration,gotze2019higher,adamczak2019note}. However, when the correlations are larger, even simple functions as $\sum_i x_i$ might not concentrate. A very strong and relatively recent approach by \citet{chatterjee2005concentration} uses Stein's method of exchangeable pairs to prove measure concentration in very general settings. As an application, he derived new concentration inequalities for the Ising model. A direct application was used to bound $\varphi'$ in prior work \cite{chatterjee2007estimation,bhattacharya2018inference,ghosal2018joint,daskalakis2019regression}, and $\varphi''$ was bounded using other techniques which were specific to the function $\varphi$ that is analyzed. We emphasize that not many techniques are known to prove concentration outside of Dobrushin's condition and Chatterjee's technique exchangeable pairs can be very challenging to apply in this regime. \nishanth{this regime meaning Dobrushin or outside Dobrushin?}

In this work, we analyze the ratio $\varphi'/\varphi''$ by a reduction from low temperature Ising models to high temperature SEC, which enables us to apply concentration inequalities that are significantly more flexible REF. This allows us to obtain more general results and remove many of the conditions required in prior work CITE, while re-deriving concentration inequalities for low temperature Ising models that were previously proven only using Chatterjee's exchangeable pairs (to the best of our knowledge).

A further contribution of this work is the following: while concentration inequalities for polynomials of high temperature Ising models were extensively studied CITE, in this work we show how to derive the same bounds on non-polynomial functions that their low-order Taylor expansion is bounded by a polynomial. We apply this inequality to bound $\varphi'$. The proof is a simple extension of CITE.

The reduction from low to high temperature is discussed in SEC, the concentration inequality is given in SEC, a proof overview is given in SEC and comparison to the techniques of prior work is given in SEC.

\subsubsection{Reducing from low to high temperature Ising models.}


\paragraph{Concentration in low temperature}
Using Lemma~\ref{lem:informal-subsample} we can re-derive inequalities that were previously proven using Chatterjee's exchangeable pair technique for concentration inequalities. One example is a bound on the derivative $\varphi'$ derived previously by Chatterjee~\cite{chatterjee2007estimation}, and another example is the following concentration inequality, for which we derive the same guarantee as Chatterjee~\cite[Proposition~3.4]{chatterjee2005concentration} up to constants.

\begin{lemma}\label{lem:curie-weiss}
	Let $x$ denote the Ising model with interaction $J_{ij} = \mathbf{1}(i\ne j)\beta/n$ (i.e. the \emph{Cury Weiss model}). Then, there exists a constant $C>0$ such that
	\[
	\Pr[|m(x) - \tanh(\beta m)| \ge \frac{\beta}{n} + t]
	\le 2\exp\left(-\frac{nt^2}{C\beta}\right).
	\]
\end{lemma}

Both inequalities are proved by deriving a concentration for functions of the form $F(x) = \sum_{i=1}^n f_i(x)$, where $f_i(x)$ is conditionally zero conditioned on $x_{-i}:= x_{[n]\setminus\{i\}}$. For a general proof approach, we will decompose $F$ into a sum of $\ell$ functions that correspond to the sets $I_1,\dots,I_\ell$ from Lemma~\ref{lem:informal-subsample}: let $F_{I_j}(x) = \sum_{i \in I_j} f_i(x)$. Then, since each $i\in[n]$ is contained in $\ell'$ sets $I_j$,
\begin{equation} \label{eq:F-decomposition}
|F(x)| = \left|\frac{1}{\ell'} \sum_{j\in [\ell]} F_{I_j}(x)\right|
\le \frac{1}{\ell'} \sum_{j\in [\ell]} \left| F_{I_j}(x) \right|
\le \frac{\ell}{\ell'} \max_{j} \left| F_{I_j}(x) \right|
\le O(1)\max_{j} \left| F_{I_j}(x) \right|.
\end{equation}
We will show that each $F_{I_j}(x)$ concentrates around zero, and this implies that $F(x)$ concentrates. It suffices to show that conditioned on any value of $x_{-I_j}$, $F_{I_j}(x)$ concentrates around zero. This is equivalent to showing that conditioned on any $x_{-I_j}$, $F_{I_j}(x)$ has zero mean and concentrates around its mean. The zero mean property follows from the fact that $f_i(x)$ is zero mean conditioned on $x_{-i}$. And the concentration property follows from the fact that $x_{I_j}$ is conditionally in high temperature, conditioned on $x_{-I_j}$: we can apply the strong concentration inequalities for Dobrushin random variables, assuming that $F_{I_j}$ satisfies their conditions, to bound $\Pr[|F_{I_j}(x)|>t \mid x_{-I_j}]$.

\paragraph{Bounding the PMLE error}
Based on the bound on the concentration inequality derivation, we describe how to bound the ratio $\varphi'(x;\beta^*)/\varphi''(x;\beta^*)$ that provides an upper bound on the error $|\hat{\beta}-\beta^*|$, and note that similar arguments may also be applied in other applications of the PMLE. First, we decompose the derivative $\varphi'(x;\beta^*) = \sum_i \varphi'_i(x)$ where $\varphi'_i(x) := -\frac{d}{d\beta}\log\Pr[x_i \mid x_{-i};\beta]\big|_{\beta=\beta^*}$. It holds that $\E[\varphi'_i(x)\mid x_{-i}] = 0$, even for arbitrary random vectors $x$.\footnote{Regularity condition ...\yuval{TODO}} Defining $\varphi'_{I_j}(x) := \sum_{i \in I_j} \varphi'_i(x)$, we will show that conditioned on each $x_{-I_j}$, $|\varphi'_{I_j}(x)| \le O(\sqrt{\varphi''(x;\beta^*)})$ with high probability. This is achieved by the following: first, we apply high-temperature concentration inequalities for $\varphi'_{I_j}(x)$; then, we show that conditioned on $x_{-I_j}$, the conditional mean of $\varphi''(x;\beta^*)$ is large. Lastly, we apply high-temperature concentration inequalities to derive that $\varphi''(x;\beta^*)$ concentrates around its mean conditioned on $x_{-I_j}$. The above derives that $|\varphi'_{I_j}(x)| \le O(\sqrt{\varphi''(x;\beta^*)})$ with high probability, and by \eqref{eq:F-decomposition} we derive that $|\varphi'(x;\beta^*)| \le O(\sqrt{\varphi''(x;\beta^*)})$, which implies that $|\hat\beta-\beta^*| \le \varphi''(x;\beta^*)^{-1/2}$. Given a lower bound on $\varphi''(x;\beta^*)$, the proof concludes. Notice that the lower bound in terms of $\|J\|_F$ is already obtained in the conditioning argument, while the bound in terms of the partition function is from CITE.

It is worth mentioning the following distinction from prior work, that derived separate bounds for $\varphi'$ and $\varphi''$: namely, they found values $\kappa_1, \kappa_2>0$, such that $|\varphi'(x;\beta^*)| \le \kappa_1$ and $\varphi''(x;\beta^*)\ge \kappa_2$, with high probability, which implies that $|\varphi'|/\varphi'' \le \kappa_1/\kappa_2$. However, this required regularity assumptions, as assuming a partition function of maximal order CITE, a Frobenius norm of maximal order CITE, or assuming that the partition function does not significantly change in a neighborhood of $\beta^*$ CITE. Without these assumptions, and outside of Dobrushin's condition, it is not clear whether such a bound is possible. In our proof, we overcome this obstacle by conditioning on a set of variables, and only show that \emph{conditionally}, the ratio $|\varphi'|/\varphi''$ is bounded.


\subsection{Organization}
\nishanth{Will be filled at the end.}




\iffalse
\subsection{Notes (To be removed eventually)}
\costis{A few things from our discussion today:
\begin{itemize}
    %\item Write a few remarks interpreting the choice of learning under Frobenius norm: namely (i) couldn't have learned in TV; (ii) conditions under which this can be used to identify the parameters of a Kernel matrix $A$ computed wrt some base distances $d(i,j)$; (iii) conditions under which the $\beta_i$'s can be identified if the $A^{(i)}$'s are sufficiently orthogonal
    \item Interesting for the future: learn in Wasserstein
    %\item In terms of techniques, illustrate: (i) conditioning trick to get Dobrushin of the conditional measure and use stronger concentration there; (ii)  concentration inequality for non-polynomials; (iii)  anti-concentration inequality for linear functions
\end{itemize}}
Pointers
\begin{enumerate}
    %\item Main motivation comes from multiple social networks: FB vs Twitter which affects political decision better.
    %\item Geographical distance motivation from Costis discussion. Don't know the right notion of distance.
    \item Does learning in Frobenius norm imply a bound on the TV? No. Add discussionc with example of distinguishing between $n$ tosses from $Ber(0)$ and $Ber(1/n)$.
    \item Highlight technical meat - throw light on the argument where you can prove that subset of vertices satisfying conditional Dobrushin always exists when the infinity norm is bounded by a constant.
    \item Highlight the anti-concentration result - Lemma 4.
    \item Need to bring out the innovation and explain potential other use cases of the technical properties.
    \item \yuval{added some pointers here.} See the second overleaf document for references.
    \item Notice that the conditioning technique can re-derive the bounds which were previously obtained using Chatterjee's exchangeable pair technique. Here we can bypass Chatterjee's technique and use directly results for high temperature.
    \item Our result holds in all temperatures: while "inference in ising models" has results for settings where the partition function is lower, it requires regularity conditions (2.6). This result, however, holds regardless. \nishanth{does this not boil down implicitly to a $1/\|A \|_F$ rate?}
    \item Emphasize simplicity of our result. Minimal and easily understandable conditions compared to prior work and also tight in many regimes.
\end{enumerate}

\yuval{Should we have a separate section containing all the relevant probabilistic results?}
\nishanth{let's take a call based on space?}\\


\yuval{Following our discussion: 
\begin{enumerate}
    \item Emphasize the cleanness of this result compared to prior work. And the fact that the condition is easy to verify and it holds even under phase transitions. Plus it's tight under Dobrushin.
    \item 
    Say why it's not straight forward to extend the prior work to multiple parameters (I will write a paragraph based on this)\\ (1) The partition function, used in "Estimation in a spinglass" and "inference in ising models" does not characterize learning multiple parameters. (2) The "joint estimation" paper has a condition specific to learning one matrix and a constant field. (3) The STOC paper reduces the task to learning one parameter, and this can only be done with multiple external field parameters and not with additional matrix parameters. (4) Chatterjee himself said that it is a challenge to extend to multiple parameters in his first paper. (5) Using only the partition function or $\Omega(n)$ norm condition (\nishanth{what is the $\Omega(n)$ norm condition?}), it is hard to guarantee that we can learn with many parameters. (6) Even the $1$-sparse setting suffers from these issues. (7) First elaborate on our improvements in the $1$-parameter settings, then show how these can lead to a simple guarantee for the sparse setting. (8) Elaborate that in prior work there were two types of results: one with Frobenius norm and one with partition function. They both are hard to generalize. (9) STOC paper relied on the fact that there are many entries with large values.
    \item More examples: (1) Can we find an example from healthcare? (2) economics blog post. \href{https://voxeu.org/article/standard-errors-persistence}{https://voxeu.org/article/standard-errors-persistence}. (3) Correlations across different countries are different. But, there are also inter-country correlations.
    \item Give an example with temporal correlations: you get multiple samples from an ising model graph which are iid-like, however, there are temporal correlations between the sampeles (plus spacial correlations within the graph). Consider both the 2-parameter variant and the multi-parameter variant.
    \item Do we want to write a result that extends the prior work? We can extend STOC paper both to: (1) learning from a few parameters. and (2) obtaining a rate which decays smoothly as the Forbenius norm decreases. And (3) can we derive results from "inference in Ising models / join estimation?" (4) Can we say anything about the partition function? 
    \item I will write a comment about why $\ell_\infty$ and not $\ell_2$. Basically, to apply it in a neat way, we need to extend the concentration result. Although the inference paper didn't have this assumption, still, it had a different condition that replaces it. And the STOC paper assumes this as well. We decided to avoid the route of inference in Ising models, to keep the proof simple.
\end{enumerate}
}
\fi

==> pgd.tex <==
\section{Projected Gradient Descent Analysis}
\label{sec:gd-analysis}
\nishanth{copied from an old paper. change to our setting.}

We will use the following well known property of Projected Gradient Descent (Theorem 3.10 from \cite{bubeck2015convex}).
\begin{theorem}\label{thm:projected} Let $f$ be $\alpha$-strongly convex and $\lambda$-smooth on compact set $\mathcal{X}$. Then
projected gradient descent with stepsize $\eta = \frac{1}{\lambda}$ satisfies for $t\geq 0$
\begin{equation}
\norm{\vec{x}_{t+1} - \vec{x}^*}_2^2 \leq e^{-\frac{\alpha t}{\lambda}}\norm{\vec{x}_{1} - \vec{x}^*}_2^2.
\end{equation}
Therefore, setting $R = \norm{\vec{x}_{1} - \vec{x}^*}_2$ and by choosing $t = \frac{2\lambda \ln \frac{R}{\epsilon}}{\alpha}$ it is guaranteed that $\norm{\vec{x}_{t+1} - \vec{x}^*}_2 \leq \epsilon$.
\end{theorem}
\subsubsection{Projected Gradient Descent for Logistic Regression}
We consider the function $LPL(\theta,\beta)$ (log-pseudolikelihood as defined in Section \ref{sec:logistic}) and we would like to approximate $(\hat{\theta},\hat{\beta})$ within $\frac{1}{\sqrt{n}}$ in $\ell_2$ distance. The stepsize in Theorem \ref{thm:projected} should be $\eta=\frac{1}{\sqrt{d\Theta^2 +1}}$ by Remark \ref{rem:smooth}.

\begin{algorithm}[H]
	\label{alg:pgd-logistic}
	\KwData{Vector sample $\vec{y}$, Magnetizations $m_i(\vec{y}) = \sum_j A_{ij}y_j$, Feature vectors $\vec{x}_i$}
	\KwResult{Maximum Pseudolikelihood Estimate}
	$\beta^0 =0, \theta^0 = \vec{0}, \textrm{normgrad} = +\infty$, $\eta = \frac{1}{\sqrt{d\Theta^2 +1}}$\;
	$t = 0$\;
	\While{$\textrm{normgrad} > \frac{1}{\sqrt{n}}$}{
		$\textrm{grad}_{\theta}=0$\;
		$\textrm{grad}_{\beta} = -\frac{1}{n}\sum_{i=1}^n \left[ y_i m_{i}(\vec{y}) -  m_i(\vec{y})\tanh (\beta^t m_i(\vec{y})+\theta^{t \;\top}\vec{x}_i)\right]$\;
		\For{$k=1;k\leq d;k++$}
		{
			$\textrm{grad}_{\theta_k} = -\frac{1}{n}\sum_{i=1}^n \left[ y_ix_{i,k} - x_{i,k}\tanh (\beta^t m_i(\vec{y})+\theta^{t \;\top}\vec{x}_i)\right]$\;
			$\textrm{grad}_{\theta} = \textrm{grad}_{\theta} + \textrm{grad}^2_{\theta_k}$\;
		}
		$\textrm{normgrad} = \sqrt{\textrm{grad}^2_{\beta}+\textrm{grad}_{\theta}}$\; 
		
		$\beta^{t+1} = \beta^t -  \eta\textrm{grad}_{\beta}$    \% update $\beta^t$\;
		\For{$k=1;k\leq d;k++$}
		{
			$\theta^{t+1}_k = \theta^t_k - \eta\textrm{grad}_{\theta_k}$     \% update $\theta^t_k$\;
		}
		$t = t+1$\;
		\% $\ell_2$ projection\\
		\If{$\beta^{t+1} <0$}{
			$\beta^{t+1} = 0$\;
		}
		\If{$\beta^{t+1} > B $}{
			$\beta^{t+1} = B $\;
		}
		\For{$k=1;k \leq d;k++$}{
			\If{$\theta^{t+1}_k < - \Theta$}{
				$\theta^{t+1}_k = -\Theta$\;
			}
			\If{$\theta^{t+1}_k > \Theta$}{
				$\theta^{t+1}_k = \Theta$\;
			}
			
		}
	}
	\Return{$(\theta^t,\beta^t)$}
	\caption{Projected Gradient Descent (Logistic)}
\end{algorithm}

==> pr-lemma-main.tex <==
\subsection{Proof of Lemma~\ref{lem:main-general}}
\label{sec:pr-lem-main}
\yuval{Not needed}

\begin{proof}[Proof of Lemma~\ref{lem:main-general}]
First, notice that 
$\|J-J^*\|_F \le \sqrt{n}\|J-J^*\|_2 \le \sqrt{n} \|J-J\|_\infty \le C\sqrt{n}$. Hence, it suffices for the proof to assume that $\sqrt{k\log n +\log(1/\delta)} = O(\sqrt{n})$.

Let
$\xi = C\sqrt{k \log n + \log(1/\delta)}$ 
and $t = C'\sqrt{k \log n + \log(1/\delta)}$, for some sufficiently large $C$ and $C'$ and, as discussed above, we can assume that $t\le \sqrt{n}$, as in the requirement of Lemma~\ref{lem:main}. Let $\Delta = \hat{J} - J^*$ and set $A = \Delta/\|\Delta\|_F$.
We begin by distinguishing between two cases. If $A \notin \mathcal{A}_\xi$, then by definition we should have
$$
\frac{\|\Delta\|_F}{\|\Delta\|_\infty} 
\le \frac{\|\Delta\|_F}{\|\Delta\|_2}
\le \xi \implies
\|\Delta\|_F \le C \sqrt{k \log n + \log(1/\delta)} \|\Delta\|_\infty.
$$
By assumption, we have
$\|\hat{J}\|_F \le M$ and $\|J^*\|_F \le M$.
We conclude that in this case
$$
\|\Delta\|_F \le 2MC\sqrt{k \log n + \log(1/\delta)}.
$$
Now suppose $A \in \mathcal{A}_\xi$.
%Then, by an application of Lemma~\ref{lem:main} we get that there
%are constants $C(M,\gamma),c'(M,\gamma)$ such that with probability
%at least $1 - \delta$ inequalities \ref{eq:main1} and \ref{eq:main2} hold.
Define the function $h:[0,\|\Delta\|_F] \mapsto \R$ such that 
$$
h(s) = \varphi(J^* + s A).
$$
By definition we have $h'(0) = \partial \varphi(J^*) / \partial A$, and also notice that
%$$
%h'(\|\Delta\|_F) = \lim_{s \to \|\Delta\|_F} \frac{\varphi(J^* + sA) - \varphi(J^* + \|\Delta\|_F A) }{s - \|\Delta\|_F}=
%\lim_{u \to 0} \frac{\varphi(\hat{J} + uA)-\varphi(\hat{J})}{u}
%= \frac{\partial \varphi(\hat{J})}{\partial A}.
%$$
%$h'(s) = \partial \varphi(J^* + sA)/ \partial A$ for all $s \in \lp[0,\|\Delta\|_F\rp]$.
$h''(s) = \partial^2 \varphi(J^* + sA)/ \partial A^2$ for all $s \in \lp[0,\|\Delta\|_F\rp]$. Those first and second derivatives are bounded in Lemma~\ref{lem:main}, and we will use them to bound $\|\hat{J} - J^*\|_F$.

Next, define the quadratic polynomial $p \colon \mathbb{R} \to \mathbb{R}$ by 
\begin{equation} \label{eq:38}
p(s)
= h(0) + h'(0) s + \frac{\mu s^2}{2}
= \frac{\mu(s+h'(0)/\mu)^2}{2} + h(0) - \frac{h'(0)^2}{2\mu}
\end{equation}
where $\mu = \inf_{s \in (0,\|\Delta\|_F)} h''(s)$. Notice that $p$ is is tangent to $h$ at $0$ and since $h$ is $\mu$-strongly convex, hence it follows that $h \ge p$ in $[0,\|\Delta\|_F]$. For all $s \in \mathbb{R}$, we use \eqref{eq:38} to extract $|s-0| = |s|$:
\[
|s+h'(0)/\mu| = \sqrt{\frac{2(p(s)-h(0))}{\mu}+ \frac{h'(0)^2}{\mu^2}}
\le \sqrt{\frac{2}{\mu}\max\left(p(s)-h(0),0\right)}+ \sqrt{\frac{h'(0)^2}{\mu^2}},
\]
by using $\sqrt{a+b} \le \sqrt{a} + \sqrt{b}$ for $a,b\ge 0$ and the fact that $s \mapsto \sqrt{s}$ is monotonic non-decreasing.
We derive that
\begin{equation}\label{eq:61}
|s| \le 2 \left|\frac{h'(0)}{\mu}\right| + \sqrt{\frac{2}{\mu}\max\left(p(s)-h(0),0\right)}.
\end{equation}
We will bound this quantity, substituting $s = \|\Delta\|_F$. First, by Lemma~\ref{lem:main},
\[
\left|\frac{h'(0)}{\mu}\right|
= \frac{\partial\psi(J^*)/\partial A}{\partial^2(J)/\partial^2 A}
\le tC \le C \sqrt{k\log n + \log(1/\delta)},
\]
where $J = J^* + s A$ for some $s \in [0,\|\Delta\|_F]$. 
Secondly, using the fact that $p$ is tangent to $h$ at $0$ and otherwise $p\le h$, we derive that
\[
p(\|\Delta\|_F) - p(0) 
\le h(\|\Delta\|_F) - h(0)
= \varphi(\hat{J}) - \varphi(J^*)
\le k,
\]
where the last inequality follows from the assumption of this lemma. We derive that
\[
\sqrt{\frac{2}{\mu}\max\left(p(s)-h(0),0\right)}
\le C \sqrt{k}.
\]
By \eqref{eq:61} we derive that $\|\Delta\|_F \le C \sqrt{k\log n + \log(1/\delta)}$ as required.
\end{proof}

\subsection{Proof for the lemma on one $J$}

\subsection{Generalizing to multiple $J$s (the main theorem)}

==> sparse-setting.tex <==
\section{Sparse setting}

The second theorem that we have is the following:
\begin{theorem}
	Let $A^1, \dots, A^k \in M_{n\times n}(\mathbb{R})$, fix $M>0$ and $s \in \mathbb{N}$, and let $\mathcal{J} := \{J = \sum_i \beta_i A^i \colon \|J\|_\infty \le M, \|\beta\|_0 \le s\}$. Then, there is an algorithm that given a sample $X$ from an Ising model with an unknown interaction matrix $J^* \in \mathcal{J}$, outputs $\hat{J}$, such that with probability $1-\delta$,
	\[
	\|J^* - \hat{J}\|_F \le \tilde O(\sqrt{k}).
	\]
	Furthermore, the algorithm runs in time $poly(n,k) \cdot n^s$.
\end{theorem}


==> techniques-old.tex <==
\subsection{Older technique stuff}

\yuval{Below has to be shortened and generalized.}

\yuval{First, show the lemma.\\ Then, show how to use it to derive concentration and link to the appendix where we apply it to the cury weiss model which are tight up to a constant (when applying, use it for functions of conditionally zero mean; Then, do union bound, and say that the log n factor can be removed).\\ Then, apply to prove lower bound for the ratio of derivatives. And take a union bound. Deriving that the derivative is bounded by the strong convexity. Say that (1) this can be generalized. and (2) that they might not concentrate.\\ A proof summary.}

It remains to show that the point $\hat{\vec{\beta}}$, which optimizes the empirical pseudo-likelihood of the model, is close to the true parameter $\vec{\beta}$ and approaches $\vec{\beta}$ as $n \to \infty$ and this is the challenging task.
Prior works show consistency of the maximum pseudo-likelihood estimator via the following two properties:
\begin{itemize}
    \item An upper bound on $\|\nabla \varphi(\beta) \|_2$ at the true parameter.
    \item A lower bound on the smallest eigenvalue of $\nabla^2 \varphi(\beta)$ in a sufficiently large region around $\hat{\beta}$.
\end{itemize}

Techniques from prior work for showing the above properties do not extend well to the setting with multiple parameters. This is because ... \nishanth{@Yuval your paragraph will plug here}. \yuval{Perhaps move it below the techniques? I would like, at the same time, to explain also how our paper resolves these.}

We take a novel approach to show the above properties of the maximum pseudo-likelihood estimator. We use strong concentration bounds on functions of the Ising model which are known under a certain weak dependence regime known as the high-temperature setting. This is characterized by a technical condition known as Dobrushin's condition (see \ref{def:dobrushin})

%1. Explain what goes wrong when trying to extend this approach to cases with small Frobenius norm. 
%2. Introduce Dobrushin's condition here and say it has nice properties which if we can port would be great.
%3. Say we introduce a novel 
%\nishanth{TODO}.


To achieve the results, we need to prove some novel properties of Ising models which we believe have potential applications outside this work. We highlight these technical vignettes below. \yuval{I am planning to connect it also with the specific proof in our paper, perhaps we need to reorganize later.}

\subsubsection{Conditioning trick} \label{sec:conditioning}
\yuval{Figure out how to merge this paragraph with the introduction on Dobrushin's condition.}
Recall that for a random variable $x$ in high temperature, many strong concentration inequalities for functions $f(x)$ are known to hold. On the other hand, if $x$ is low temperature, even very basic functions as $\sum_i x_i$ may not concentrate. Even if they do, there are not many tools to prove that.
Hence, we would like to utilize the high temperature concentration inequalities, even for low temperature distributions.
In order to achieve that, notice that if we condition on a large subset of the variables, the remaining variables can be conditionally high temperature. The most fundamental example is when $J$ is the incidence matrix of a bipartite graph, namely, there exists a set $I \subseteq [n]$ such that $J_{ij} = 0$ whenever either $i,j\in I$ or $i,j\in [n]\setminus I$ (this model is also called a \emph{Boltzman machine}). If we condition on $x_{-I} := x_{[n]\setminus I}$, then $\{x_i \colon i \in I\}$ are conditionally independent. For general Ising models with bounded $\|J\|_\infty$, we show a systematic way to condition on a subset of the variables to obtain a conditionally Dobrushin random variable. Then, we demonstrate how they can be used to prove properties of the Ising model, sketching examples from the proof of Theorem~\ref{thm:informal-main}. We start with the conditioning lemma:
\begin{informallemma} \label{lem:informal-subsample}
	Let $x$ be an Ising model with interaction matrix $J$ satisfying $\|J\|_\infty = M$. Then there exist $\ell=O(\log n)$ sets $I_1,\dots,I_\ell \subseteq [n]$ such that:
	\begin{enumerate}
		\item Each $i\in I$ appears in exactly $\ell'=\lceil\ell/(16M)\rceil$ different sets $I_j$.
		\item For all $j \in [\ell]$, $x_{I_j}$ is conditionally Dobrushin with coefficient $\alpha=1/2$, conditioned on $x_{-I_j}$.
	\end{enumerate}
\end{informallemma}
The sets are constructed randomly using a simple combinatorial trick that could be found in \cite{alon2004probabilistic}. \yuval{move the proof outline to a section below?} The main idea is to draw independent random subsets $\{I_j' \colon j \in [\ell]\}$, and then remove from $I_j'$ all the coordinates $i$ that have many neighbors within $I_j'$, namely, $I_j = \{i \in I_j' \colon \sum_{i'\in I_j'} |J_{ii'}| \le 1/2\}$. We can show that with high probability, each $i \in [n]$ is contained in at least $\ell'$ sets, and then remove $i$ from some of the sets to satisfy the first requirement of the lemma. This suffices, since the second requirement trivially holds.

\yuval{Find out the concentration inequality from Chatterjee's thesis that he said that he doesn't think was known before of his exchangeable pair technique.}

\begin{remark}
	\yuval{Modify in accordance to whether Dobrushin's condition for general distributions is mentioned above. Perhaps remove this.}
	For random vectors $x=(x_1,\dots,x_n)$ over general domains, one can define an \emph{independence matrix} $J$ that captures pairwise influences between the coordinates of $x$, thereby generalizing the notion of interaction matrix. In this setting, Dobrushin's condition holds whenever $\|J\|_\infty < 1$, and analogously, Lemma~\ref{lem:informal-subsample} can be applied as a tool to reduce $\|A\|_\infty$ below $1$.
\end{remark}

\paragraph{Anti concentration inequality for linear functions}

As a first application to this technique, given a vector $a \in \mathbb{R}^n$, we would like to lower bound the variance of $a^\top x$. It is well known that if $x$ is an $i.i.d.$ vector of binary random variables, each with variance $v$, then $\Var(a^\top x) = v\|a\|_2^2$. Furthermore, if $x$ has a low Dobrushin's coefficient, we can also show that $\Var(a^\top x) \ge \Omega(\|a\|_2^2)$, using the fact that its covariance matrix is diagonally dominant. We will use Lemma~\ref{lem:informal-subsample} to show that a similar lower bound holds even outside of Dobrushin's condition:
\begin{informallemma}
	Let $x$ be a random variable with interaction matrix satisfying $\|J\|_\infty = O(1)$ and bounded external field, $\|h\|_\infty = O(1)$. Then, for all $a \in \mathbb{R}^n$,
	\[
	\Var(a^\top x) \ge \Omega(\|a\|_2^2).
	\]
\end{informallemma}
To prove this lemma, consider the sets $I_1,\dots,I_\ell$ from Lemma~\ref{lem:informal-subsample}. First, we claim that there exists $j \in [\ell]$ such that $\|a_{I_j}\|_2^2 \ge \Omega(\|a\|_2^2)$. Indeed, by linearity of expectation, if we draw $j \in [\ell]$ uniformly at random then,
\[
\E_j[\|a_{I_j}\|_2^2]
= \E\left[\sum_{i=1}^n \mathbf{1}(i \in I_j) a_i^2\right]
= \sum_{i=1}^n \frac{\ell'}{\ell} a_i^2
= \frac{\ell'}{\ell}\|a\|_2^2
\ge \Omega(\|a\|_2^2).
\]
Hence, there exists a set $I_j$ that achieves this expectation, namely, $\|a_{I_j}\|_2^2 \ge \Omega(\|a\|_2^2)$. Therefore, we can bound $\Var[a^\top x \mid x_{-I}] \ge \Omega(\|a_I\|_2^2)$ 
and conclude that
\[
\Var(a^\top x) 
\ge \E_{x_{-I}}[\Var[a^\top x | x_{-I}]] 
\ge \Omega(\|a_I\|_2^2)
\ge \Omega(\|a\|_2^2).
\]

\paragraph{Concentration inequalities}

Next, we show how to apply Lemma~\ref{lem:informal-subsample} in combination with concentration inequalities for Dobrushin random variables, to prove concentration results in low temperature. In fact, this will re-derive inequalities by Chatterjee~\cite[Proposition~3.4]{chatterjee2005concentration} and \cite{chatterjee2007estimation}, that were previously proven only using his exchangeable pairs technique, as far as we are aware of. The inequality from \cite{chatterjee2007estimation} bounds the derivative of the log pseudo likelihood, and was used in all prior work \cite{daskalakis2018efficient,bhattacharya2018inference,ghosal2018joint,chatterjee2007estimation}. Due to reasons explained in the next paragraph, we could not use the exchangeable pair technique for the purpose of this paper.

As a starting point, assume that $f_1,\dots,f_n$ are real functions of $(x_1,\dots,x_n)$, such that $\E[f_i\mid x_{-i}] = 0$ for all $i$. Our goal is to show tail bounds for $F(x) := \sum_i f_i(x)$. A common route is to bound $\|F(x)\|_p := \E[F(x)^p]^{1/p}$ and apply Markov's inequality on $F(x)^p$. It is worth noting that $\|F(x)\|_p \le \sqrt{Kp}$ holds for all $p \ge 1$ if and only if $\Pr[|F(x)|>t] \le 2\exp(-t^2/(CK))$ holds for all $t > 0$, where $C>0$ is a small constant.
\begin{lemma}\label{lem:informal-concentration}
	Let $x$ be an Ising model with interaction matrix $J$. Let $I_1,\dots,I_\ell$ denote the sets from Lemma~\ref{lem:informal-subsample}, let $F(x):= \sum_{i=1}^n f_i(x)$ for some functions $f_i$ and let $F_{I_j}(x) :=\sum_{i \in I_j} f_i(x)$. Then, for any $p\ge 1$,
	\[
	\|F(x)\|_p
	\le (16\|J\|_\infty \max_{j \in [\ell]} \|F_{I_j}(x)^p\|
	\le 16\|J\|_\infty\max_{j \in [\ell]}\max_{u_{-I_j} \in \{-1,1\}^{n-|I_j|}} \E\left[F_{I_j}(x)^p ~\middle|~ x_{-I_j} = u_{-I_j}\right]^{1/p}.
	\]
\end{lemma}
\begin{proof}
	While the second inequality is trivial, we will prove the first inequality.
	Recall that each $i \in [n]$ appears in exactly $\ell' := \lceil \ell/(16\|J\|_\infty)\rceil$ different sets $I_j$. Then,
	$F(x) = \frac{1}{\ell'} \sum_{j \in [\ell]}F_{I_j}(x)$. Hence, using Minkowsky's inequality, we obtain that 
	\[
	\|F(x)\|_p \le \frac{1}{\ell'}\sum_j \|F_{I_j}(x)\|_p \le 
	\frac{\ell}{\ell'}\max_j \|F_{I_j}(x)\|_p
	\le 16\|J\|_\infty\max_j \|F_{I_j}(x)\|_p.
	\]
\end{proof}

In order to apply the above lemma, it suffices to use concentration inequalities for $F_{I_j}:=\sum_{i\in I_j}f_i(x)$, while conditioning on $x_{-I_j}$. Since $x_{I_j}$ is conditionally Dobrushin it will be easier to obtain such bounds. If we assume that $f_i$ has zero mean conditioned on $x_{-i}$, then $F_{I_j}$ has zero mean conditioned on $x_{-I_j}$, hence, one only has to argue about deviation from the mean to bound $F_{I_j}(x)^p$.

Here we apply Lemma~\ref{lem:informal-concentration} to the first inequality discussed above \cite[Proposition~3.4]{chatterjee2005concentration} while the second inequality \cite{chatterjee2007estimation} is very similar. Define the \emph{Curie Weiss} as the Ising model with interaction matrix $J$, where $J_{ij} = \frac{\beta}{n}\mathbf{1}_{i\ne j}$, for $\beta\in \mathbb{R}$. The following lemma bounds the concentration of the \emph{magnetization} $m(x) := \sum_i x_i/n$, deriving a the same guarantee as \cite{chatterjee2005concentration} up to constant factors.\footnote{We omitted the external field $h$ appearing in \cite{chatterjee2007estimation} for simplicity.} The proof follows similar structure to \cite{chatterjee2005concentration}, while replacing the exchangeable pair technique with Lemma~\ref{lem:informal-concentration} together with concentration under Dobrushin, and omitting some calculations.
\begin{lemma}\label{lem:curie-weiss}
	Let $x$ denote the Currie Weiss model. Then, there exists a constant $C>0$ such that
	\[
	\Pr[|m(x) - \tanh(\beta m)| \ge \frac{\beta}{n} + t]
	\le 2\exp\left(-\frac{nt^2}{C\beta}\right).
	\]
\end{lemma}
Before proving Lemma~\ref{lem:curie-weiss}, we state McDiarmid's inequality for high temperature Ising models, which has the same guarantees as for independent random variables, up to constants \yuval{Find a citation older than Chatterjee's (the older the better)}:
\begin{proposition}\label{prop:McDiarmid}
	Let $y \in \{-1,1\}^m$ be a high temperature Ising model and let $g(y)$ be a real function satisfying $\lambda$-bounded differences, namely, $|g(y)-g(y')|\le \lambda$ whenever $y$ and $y'$ differ on one coordinate. Then, for any $p \ge 1$, $\E[(g(y)-\E g(y))^p]^{1/p} \le C \lambda\sqrt{mp}$.
\end{proposition}
\begin{proof}[Proof sketch of Lemma~\ref{lem:curie-weiss}]
	For simplicity, assume that $\beta > 1$. Let $m_i(x) = \sum_{j\ne i} x_j/n$. We will bound $F(x) :=\sum_i f_i(x)$ where $f_i(x) = (x_i - m_i(x))/n$ and this will suffice since $|m-\tanh(\beta n) - F(x)| \le \beta/n$.
	Applying Lemma~\ref{lem:informal-concentration}, we obtain that
	\[
	\E[F(x)^p]
	\le (16\|J\|_\infty)^p\max_{j \in [\ell]}\max_{u_{-I_j} \in \{-1,1\}^{n-|I_j|}} \E\left[F_{I_j}(x)^p ~\middle|~ x_{-I_j} = u_{-I_j}\right].
	\]
	In this application it would suffice to take $I_j$ to be disjoint sets, each of size approximately $n/(2\beta)$, and notice that they satisfy the guarantees of Lemma~\ref{lem:informal-subsample}.
	Fix $j \in [\ell]$ and condition on $x_{-I_j} = u_{-I_j}$. Notice that conditionally, $F_{I_j}(x)$ is a function on $Cn/\beta$ variables, and since $\tanh$ is $1$-Lipschitz, $F_{I_j}(x)$ is $O(1/n)$-bounded differences. Using McDiarmid's inequality and the fact that $F_{I_j}$ is conditionally zero mean, we derive that
	\[
	\E[F_{I_j}(x)^p\mid x_{-I_j}]^{1/p} \le C\sqrt{p/(\beta n)}.
	\]
	By Lemma~\ref{lem:informal-concentration}, we have 
	\[
	\E[F(x)^p]^{1/p} \le C \|J\|_\infty \sqrt{p/(\beta n)} = O(\sqrt{p\beta/n}).
	\]
	This is equivalent to $\Pr[|F(x)|>t] \le 2\exp(-t^2 n/(C\beta))$, as required.
\end{proof}


\paragraph{Bounding the pseudo log likelihood in general settings.}
\yuval{Sell this, perhaps even in the abstract, as a technique to bound bound the PMLE in related estimation tasks. This means that we should have many citations of papers using the PMLE.}
The PMLE has been used successfully in many estimation tasks \yuval{name a few and add citations. Add some papers about triangle finding, because the theory community likes it.} Here, we show how to use Lemma~\ref{lem:informal-subsample} as a tool to analyze this estimate, while reducing the correlations by conditioning. We believe that it may have applications outside of this work, perhaps also for applications of the PMLE for non Ising models.

We make some simplifications and ignore some details in order to facilitate the presentation, focusing on one-parameter distributions: let $\Theta$ denote a family of parameter values, and let $\{P_\theta \colon \theta \in \Theta \}$ denote a family of distributions parameterized by $\theta \in \Theta$. Define the negative pesudo log likelihood estimator as
\begin{equation} \label{eq:PMLE}
\varphi(x;\theta) := \sum_{i \in [n]} \varphi_i(x;\theta) := -\sum_{i\in [n]} \log \Pr_{\theta}[x_i | x_{-i}].
\end{equation}
Let $\theta^*$ denote the true parameter, $\hat{\theta}$ is the PMLE, $\varphi'$ and $\varphi''$ denote the first and second derivatives of $\varphi$ with respect to $\theta$. When $\varphi$ is convex, a standard bound for the error is given by
\begin{equation}\label{eq:11}
|\hat\theta - \theta^*|^2 \lessapprox \frac{
	\varphi'(x;\theta^*)^2}{
	\varphi''(x;\theta^*)^2}
	\lessapprox \frac{
	\Var[\varphi'(x;\theta^*)]}{
	\varphi''(x;\theta^*)^2}
\end{equation}
where the inequalities hold up to a constant\footnote{To be concise, one should replace $\varphi''(x;\theta^*)^2$ with $\min_\theta \varphi''(x;\theta)^2$, where the minimum is taken over some neighborhood of $\theta^*$. In this paper those two quantities are nearly the same, and it is simple to make the modification if this is not the case.} and the last inequality holds with high probability since 
$\E_{\theta^*}[\varphi'(x;\theta^*)] = 0$.
Upper bounding \eqref{eq:11} amounts to showing that $\varphi'$ is close to zero, while showing that with high probability, $\varphi''$ is bounded away from zero, which amounts to showing that $\Var(\varphi'') \ll \E[\varphi'']^2$.
Since there may be strong dependencies in $x$, it may be hard to estimate these quantities. Hence, we will instead estimate the conditioned variances, while fixing some of the coordinates.
\begin{informallemma}\label{lem:informal-PMLE}
	Let $I_1,\dots,I_\ell$ denote the sets guaranteed from Lemma~\ref{lem:informal-subsample} with $\ell = O(\log n)$, and assume that for all $j \in [\ell]$ and any fixed value of $x_{-I_j}$, 
	\begin{equation} \label{eq:333}
	\Var_{\theta^*}[\varphi''(x;\theta^*) | x_{-I_j}] \ll \E_{\theta^*}[\varphi''(x;\theta^*) | x_{-I_j}]^2 / \log n.
	\end{equation}
	Let $\varphi_{I_j}'(x;\theta^*) := \sum_{i \in I_j}\varphi_{i}'(x;\theta^*)$.
	Then, with high probability,
	\[
	\frac{
		\varphi'(x;\theta^*)^2}{
		\varphi''(x;\theta^*)^2}
	\lessapprox O(\log n) \frac{\max_{j \in [\ell]}
		\Var_{\theta^*}[\varphi'_{I_j}(x;\theta^*)|x_{-I_j}]}{
		\max_{j \in [\ell]}\E_{\theta^*}[\varphi''(x;\theta^*) | x_{-I_j}]^2
	}.
	\]
	(Modifications can be made when \eqref{eq:333} does not hold for all $I_j$ and when one wants to calculate high probability rather than variance bounds. See the proof of Theorem~\ref{thm:informal-main}.)
\end{informallemma}
In order to check the conditions of Lemma~\ref{lem:informal-PMLE} we can now condition on $x_{-I_j}$, and make all the calculations with the conditioned probabilities. Apart from being easier to prove concentration inequalities in the conditioned regime, there is another advantage of this technique: it might be impossible to obtain the correct bound on $\varphi'/\varphi''$ using only the global (unconditioned) variance bounds. Namely, it can be the case that both $\varphi'$ and $\varphi''$ have large variances, however, it is almost always true that $\varphi'/\varphi''$ is bounded. Such a phenomena can occur when the distribution has multiple clusters, namely, when it can be viewed as a mixture of multiple distributions, $D_1, \dots, D_m$, each with distinct properties. In this case, $\varphi'$ and $\varphi''$ can have a different behavior for each $D_i$. However, $\theta^*$ can be learned conditioned on each cluster, and $\varphi'/\varphi''$ is small in all of them. Clusters are apparent in low temperature Ising models, and a fundamental example is the \emph{Curie Weiss} model, with interaction matrix $J_{ij} = \beta/n$ for all $i\ne j$, where $\beta > 1$. There are two clusters, one with $\sum_i x_i/n \approx a$ and the other with $\sum_i x_i/n \approx -a$, where $\{\pm a\}$ are the solution to $x = \tanh(\beta x)$. Notice that by conditioning on $x_{-I}$, one essentially fixes the cluster. Hence, conditioning will guarantee that we are comparing $\varphi'$ and $\varphi''$ within the same cluster.

In the proof of Theorem~\ref{thm:informal-main}, we use a variant of Lemma~\ref{lem:informal-PMLE}, and there, as discussed above, we show that the ratio $\varphi'/\varphi''$ is bounded with high probability over $x$, rather than treating those derivatives separately. It might still be possible to derive the correct bounds analyzing $\varphi'$ and $\varphi''$ separately: although functions of $x$ might not concentrate in low temperature, it might be the case that $\varphi'$ and $\varphi''$ do. However, we believe that in complex settings as the multi parameter learning problem or in some other related problems they may not concentrate. Lastly, we prove Lemma~\ref{lem:informal-PMLE}:
\begin{proof}[Proof sketch of Lemma~\ref{lem:informal-PMLE}]
	First, we notice that for any $j$ and any fixed value for $x_{-I_j}$, $\E[\varphi'_{I_j}(x;\theta^*) | x_{-I_j}] = 0$ \yuval{Ref to the proof}. Hence, by Markov's inequality, we get that conditioned on $x_{-I_j}$, 
	\begin{equation}\label{eq:520}
	\varphi'_{I_j}(x;\theta^*)^2
	\le \E[\varphi'_{I_j}(x;\theta^*)^2\mid x_{-I_j}] O(\log n)
	= \Var[\varphi'_{I_j}(x;\theta^*)\mid x_{-I_j}] O(\log n)
	\end{equation}
	holds with probability of at least $1-1/(C \log n)$
	where $C$ is an arbitrarily large constant.
	Let $E_j$ denote the event that \eqref{eq:520} holds for the set $I_j$, and notice that using \eqref{eq:520}, $\Pr[E_j] = \E_{x_{-I_j}}[\Pr[E_j|x_{-I_j}]] \ge 1-1/(C\log n)$.
	Next, by assumption \eqref{eq:333} we can derive that for any $j \in [\ell]$ and conditioned on $x_{-I_j}$, with probability of at least $1/(C\log n)$,
	\begin{equation}\label{eq:521}
	\varphi''(x;\theta^*) \ge \mathbb{E}_{\theta^*}[\varphi''(x;\theta^*)\mid x_{-I_j}]/2.
	\end{equation}
	Let $E'_j$ denote the event that \eqref{eq:521} holds, and notice that $\Pr[E'_j] \ge 1-1/(C\log n)$. By a union bound over $2\ell = O(\log n)$ events, $\Pr[\bigcup_j (E_j \cup E_j')]\ge 1-\delta$, where $\delta>0$ can be an arbitrary small constant. Assume next that all these events hold. Since each $i \in [n]$ is contained in exactly $\ell'$ different sets $I_j$,
	\[
	\varphi'(x;\theta^*)^2 = \left(\frac{1}{\ell'}\sum_{j \in [\ell]} \varphi_{I_j}'(x;\theta^*)\right)^2
	\le \left(\frac{\ell}{\ell'}\right)^2
	\max_{j \in [\ell]} \varphi_{I_j}'(x;\theta^*)^2
	\le \max_{j \in [\ell]}\Var[\varphi'_{I_j}(x;\theta^*)\mid x_{-I_j}] O(\log n),
	\]
	using the fact that $\ell/\ell' = O(1)$. Additionally, from \eqref{eq:521}, $\varphi''(x;\theta^*) \ge \max_{j\in [\ell]}\mathbb{E}_{\theta^*}[\varphi''(x;\theta^*)\mid x_{-I_j}]/2$, which concludes the proof.
\end{proof}



\paragraph{Older stuff 2}
\cite{chatterjee2007estimation} uses the method of exchangeable pairs to bound the variance of certain functions. Since the model does not satisfy Dobrushin's condition, generic variance bounds cannot be shown on arbitrary functions easily and arguments specific to the function under consideration are required.  A Corollary of our technical novelty is a variance bound of the same order which can be shown using the results which are known to hold under Dobrushin's condition (\ref{lem:?}).

\nishanth{Zoom discussion:
Techniques
------------
Nishanth: that is Dobrushin's condition
Yuval: what we do to reduce the setting + anti-concentration of linear functions
Vardis: concentration inequality for non-polynomial functions
Yuval: why multi-parameters is not easily implied from prior work
}

==> temp-additional-lemmas.tex <==
\section{Temporary additional lemmas}

